KGLiDS: A Platform for Semantic Abstraction, Linking, and Automation of Data Science

In recent years, we have witnessed the growing interest from academia and industry in applying data science technologies to analyze large amounts of data. In this process, a myriad of artifacts (datasets, pipeline scripts, etc.) are created. However, there has been no systematic attempt to holistically collect and exploit all the knowledge and experiences that are implicitly contained in those artifacts. Instead, data scientists recover information and expertise from colleagues or learn via trial and error. Hence, this paper presents a scalable platform, KGLiDS, that employs machine learning and knowledge graph technologies to abstract and capture the semantics of data science artifacts and their connections. Based on this information, KGLiDS enables various downstream applications, such as data discovery and pipeline automation. Our comprehensive evaluation covers use cases in data discovery, data cleaning, transformation, and AutoML. It shows that KGLiDS is significantly faster with a lower memory footprint than the state-of-the-art systems while achieving comparable or better accuracy.

==> figures/transformation.tex <==
% \begin{figure}
%     \begin{subfigure}{.67\linewidth}  % Adjust the width as needed
%         \includegraphics[width=\linewidth]{figures/transformation_autolearn.png} % Include your first image
%         \caption{Caption for the first image}
%         \label{fig:sub1}
%     \end{subfigure}%
%     \begin{subfigure}{.33\linewidth}  % Adjust the width as needed
%         % Your table here
% \begin{tabular}{lrrrrrlr}
% \hline
% Dataset&\multicolumn{3}{|c|}{Linear Regression}  & \multicolumn{3}{c|}{Random Forest} \\
% \hline
% & Baseline & Autolearn& OURS&Baseline & Autolearn& OURS& \\
% Fertility Diagnosis&88.0&&87.0 & 87.0& \\
% haberman&74.48&  & 67.66 &  67.67 &  & 67.66 \\ wine&94.41&  & 98.33 &  98.33 & 97.77& 98.33 \\ Ecoli&72.07&  & 82.11 &  86.6  &   & 82.11 \\ pima diabetes &77.09&  & 76.7  &  76.56 &   & 76.7  \\ Dermatology(mv)&97.82&  & 97.82 &  97.27 &   & 97.82 \\ Banke Note&98.98&  & 98.69 &  99.05 & 99.93& 98.69 \\ ionosphere &87.17&  & 92.3  &  93.15 & 92.33& 92.3  \\ sonar &77.98&  & 83.67 &  84.17 & 80.71& 83.67 \\ Abalone &26.02&  & 24.95 &  24.78 &   & 24.95 \\ libras&67.78&  & 79.44 &  81.39 & 81.78& 79.44 \\ waveform      &87.12&  & 85.04 &  85.26 & 79.02& 85.04 \\ letter recognition&76.07&  & 96.65 &  96.65 &   & 96.65 \\ opticaldigits &96.83&  & 98.24 &  98.19 &   & 98.24 \\ featurepixel &96.3 &  & 97.85 &  97.9  &   & 97.85 \\ shuttle         &92.05&  & 99.96 &  99.99 &   & 99.96 \\ featurefourier&81.25&  & 83    &  83.5  &  & 83    \\ poker&50.12&  & 76.08 &  76.07 & & 76.08 \\
% \hline
% \end{tabular}
%         \caption{Caption for the table}
%         \label{fig:sub2}
%     \end{subfigure}
%     \caption{Main caption for the entire figure}
%     \label{fig:main}
% \end{figure}

% \begin{figure*}[t]
%   \centering
%    \includegraphics[width=2\columnwidth]{figures/transformation_autolearn.png}
%   % \subfigure{\includegraphics[width=0.25\linewidth]{figures/exp_data_transformation_effectiveness.pdf}}\hspace{-0.10cm}
%   % \subfigure{\includegraphics[width=0.75\linewidth]{figures/exp_data_transformation_efficiency.pdf}}
%   \ncp\ncp\ncp\ncp
%   % \vspace*{-3ex}
%   \caption{Data Transformation: the performance of {\sysname} vs. existing systems on multiple ML tasks on 13 datasets. (a) in the radar diagram, the outer numbers indicate  different dataset IDs and the ticks inside the figure denote performance ranges of respective metrics, e.g., 0.2, 0.4, ..., etc. for F1 in each ML task per dataset. For any dataset, the system with the outermost curve has the best performance. {\sysname} outperforms \lfe{} and \autolearn{} in most cases. (b) and (c) the time and memory consumed per system to perform data transformation on the dataset and train the model. F1 scores of LFE are reported by the authors, but its code is not available. {\sysname} outperforms \autolearn{} in terms of time and memory performance.}
%   \label{fig:exp_data_transformation}
%   % \ncp\ncp
%   % \vspace*{-1ex}
% \end{figure*}

% \begin{figure}[htbp]
%     \begin{minipage}{0.33\textwidth}
%     \resizebox{\textwidth}{!}{
%         \begin{tabular}{lrrrrrlr}
% \hline
% Dataset&\multicolumn{3}{|c|}{Linear Regression}  & \multicolumn{3}{c|}{Random Forest} \\
% \hline
% & Baseline & Autolearn& OURS&Baseline & Autolearn& OURS& \\
% Fertility Diagnosis&88.0&&87.0 & 87.0& \\
% haberman&74.48&  & 67.66 &  67.67 &  & 67.66 \\ wine&94.41&  & 98.33 &  98.33 & 97.77& 98.33 \\ Ecoli&72.07&  & 82.11 &  86.6  &   & 82.11 \\ pima diabetes &77.09&  & 76.7  &  76.56 &   & 76.7  \\ Dermatology(mv)&97.82&  & 97.82 &  97.27 &   & 97.82 \\ Banke Note&98.98&  & 98.69 &  99.05 & 99.93& 98.69 \\ ionosphere &87.17&  & 92.3  &  93.15 & 92.33& 92.3  \\ sonar &77.98&  & 83.67 &  84.17 & 80.71& 83.67 \\ Abalone &26.02&  & 24.95 &  24.78 &   & 24.95 \\ libras&67.78&  & 79.44 &  81.39 & 81.78& 79.44 \\ waveform      &87.12&  & 85.04 &  85.26 & 79.02& 85.04 \\ letter recognition&76.07&  & 96.65 &  96.65 &   & 96.65 \\ opticaldigits &96.83&  & 98.24 &  98.19 &   & 98.24 \\ featurepixel &96.3 &  & 97.85 &  97.9  &   & 97.85 \\ shuttle         &92.05&  & 99.96 &  99.99 &   & 99.96 \\ featurefourier&81.25&  & 83    &  83.5  &  & 83    \\ poker&50.12&  & 76.08 &  76.07 & & 76.08 \\
% \hline
% \end{tabular}
% }
%         \caption{Your Table Caption}
%         \label{tab:your-table}
%     \end{minipage}
%      \hfill
%         \begin{minipage}{0.67\textwidth}
%         \includegraphics[width=\textwidth]{figures/transformation_autolearn.png}
%         \caption{Your Figure Caption}
%         \label{fig:your-figure}
%     \end{minipage}%

% \end{figure}


\begin{figure*}[htbp]
    \begin{minipage}{0.33\textwidth}
        \resizebox{\textwidth}{!}{
            \begin{tabular}{lrrrrrlr}
                \hline
                Dataset & \multicolumn{3}{|c|}{Linear Regression} & \multicolumn{3}{c|}{Random Forest} \\
                \hline
                & Baseline & Autolearn & OURS & Baseline & Autolearn & OURS & \\
                Fertility Diagnosis&88.0&&87.0 & 87.0& \\
haberman&74.48&  & 67.66 &  67.67 &  & 67.66 \\ wine&94.41&  & 98.33 &  98.33 & 97.77& 98.33 \\ Ecoli&72.07&  & 82.11 &  86.6  &   & 82.11 \\ pima diabetes &77.09&  & 76.7  &  76.56 &   & 76.7  \\ Dermatology(mv)&97.82&  & 97.82 &  97.27 &   & 97.82 \\ Banke Note&98.98&  & 98.69 &  99.05 & 99.93& 98.69 \\ ionosphere &87.17&  & 92.3  &  93.15 & 92.33& 92.3  \\ sonar &77.98&  & 83.67 &  84.17 & 80.71& 83.67 \\ Abalone &26.02&  & 24.95 &  24.78 &   & 24.95 \\ libras&67.78&  & 79.44 &  81.39 & 81.78& 79.44 \\ waveform      &87.12&  & 85.04 &  85.26 & 79.02& 85.04 \\ letter recognition&76.07&  & 96.65 &  96.65 &   & 96.65 \\ opticaldigits &96.83&  & 98.24 &  98.19 &   & 98.24 \\ featurepixel &96.3 &  & 97.85 &  97.9  &   & 97.85 \\ shuttle         &92.05&  & 99.96 &  99.99 &   & 99.96 \\ featurefourier&81.25&  & 83    &  83.5  &  & 83    \\ poker&50.12&  & 76.08 &  76.07 & & 76.08 \\
                \hline
            \end{tabular}
        }
        %\caption{(a)}
        \label{tab:your-table}
    \end{minipage}%
    \hfill
    \begin{minipage}{0.67\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/transformation_autolearn.png}
        
        \label{fig:your-figure}
    \end{minipage}
    \caption{Data Transformation: the performance of {\sysname} vs. existing systems on multiple ML tasks on 13 datasets. (a) in the radar diagram, the outer numbers indicate  different dataset IDs and the ticks inside the figure denote performance ranges of respective metrics, e.g., 0.2, 0.4, ..., etc. for F1 in each ML task per dataset. For any dataset, the system with the outermost curve has the best performance. {\sysname} outperforms \lfe{} and \autolearn{} in most cases. (b) and (c) the time and memory consumed per system to perform data transformation on the dataset and train the model. F1 scores of LFE are reported by the authors, but its code is not available. {\sysname} outperforms \autolearn{} in terms of time and memory performance.}
\end{figure*}








==> sections/applications.tex <==

\section{{\sysname}'s Automation for Data Science}
\label{sec:applications}

Due to limited space, this section focuses on our GNN models for unseen datasets to predict a data cleaning or transformation operation and select an ML classifier with its near-optimal parameters (AutoML).   


\input{sections/dataPreparation}


\begin{figure}
\vspace*{-2ex}
 \centering
  \includegraphics[width=\columnwidth]{figures/kglids_integration_with_kgpip.pdf} 
  \vspace*{-2ex}
  \caption{Changes to the KGpip AutoML system components when integrating {\sysname} for graph generation and initial hyperparameter recommendation. The green component is newly added, while the orange component is modified.}
  \label{fig:kglids_integration_with_kgpip}
  \vspace*{-2ex}
\end{figure}

\subsection{Our AutoML Support as a GNN Graph Generation Model}
\label{sec:automl_use_case}

Automated Machine Learning (AutoML) is the process of automatically generating optimized machine learning models for unseen datasets. It involves an exhaustive search over a large space to find the best scoring combination of data preprocessors, machine learning algorithms, and their corresponding hyperparameters. 
To show the usability of the {\graphname} for AutoML, we integrated {\sysname} with KGpip \cite{kgpip}, a state-of-the-art AutoML system based on graph neural networks (GNNs). Figure \ref{fig:kglids_integration_with_kgpip} shows the components of the KGpip system and the improvements provided by {\sysname}. The offline training phase of KGpip involves mining a large set of Python ML pipelines, generating pipeline graphs using GraphGen4Code\cite{graph4code}, applying an extensive graph filtration process, and training a generative graph neural network that models the distribution of pipeline graphs. The inference phase includes using the trained GNN to generate pipeline graphs, validating the top-k graphs to extract preprocessors and estimators, and using a hyperparameter optimizer to search for the best hyperparameters for the top-k preprocessors and estimators.

{\sysname} improves the KGpip system in two ways. First, the {\graphname} graph provides a more accurate and rich representation of pipeline graphs than GraphGen4Code\footnote{The development of {\sysname} is inspired by our study in the KGpip system.}, therefore improving the modeling capability of the GNN. Second, since the {\graphname} contains links between similar datasets and their pipelines, it can be queried during the inference phase for an initial configuration of hyperparameters based on the experience of data scientists. The KGpip system uses these recommendations as starting points for the hyperparameter search on unseen datasets to significantly reduce the
search time as opposed to data-independent starting points. In Section \ref{sec:evaluation}, we show that integrating {\sysname} leads to a significant improvement in the accuracy of the KGpip AutoML system.





% \subsection{Table Union Search}
% \label{sec:table_union_search_use_case}


% % \begin{figure}[t]
% %  \centering
% %   \includegraphics[width=\columnwidth]{figures/unionability_query.pdf} 
% %   \caption{A graph query in SPARQL to discovery unionable tables in the {\graphname} graph. \textbf{\texttt{TABLE\_NAME}} is the name of the query table and \textbf{\texttt{unionScore}} is the unionability score for each result table.}
% %   \label{fig:unionability_query}
% % \end{figure}

% Table union search is the task of finding tables within a data lake that can be unioned with a query table to extend it with more rows. Table union search is an essential task for data scientists given the growth in size for both open and enterprise data lakes. Existing table search approaches employ various techniques such as vector similarity search over hand-crafted features \cite{d3l}, matching tables to concepts in open or synthesized knowledge bases \cite{santos}, among others. We demonstrate that the {\graphname} graph can be utilized to build a competitive unionable table discovery system. In {\sysname}, two types of column-level relationships exist: i) label similarity exists between columns with similar names based on word embedding similarity, and ii) content similarity exists between columns with similar raw values based on their computed column embeddings. In addition, column similarity relationships exist only between columns having the same fine-grained data type.

% We leverage these relationships to determine column unionability as follows: two columns are unionable if they have \textit{both} label and content similarities with a similarity score above a user-defined threshold. Consequently, two tables are unionable if they have one or more unionable columns. Furthermore, the table unionability score is defined as the sum of the individual similarity scores between the columns. This can be expressed as the graph query shown in Figure \ref{fig:unionability_query}. Implementing unionable table discovery as a graph query offers a significant improvement in scalability over other approaches because they leverage the constructed graph indices built automatically by graph engines. In Section \ref{sec:evaluation}, we compare our method of table union search with the state-of-the-art systems in terms of accuracy and scalability.

==> sections/automationOnDemand-Khaled.tex <==
\section{On-Demand Automation in Data Science}
\label{sec:applications}

Several ML models could be developed using \sysname{} to automate different aspects of data science. The training dataset for these models is the semantics of the dataset associated with their pipeline scripts and is represented in the LiDS graph. This training dataset is significantly smaller than the raw dataset in its original format; furthermore, its graph representation makes it easier to use than heterogeneous raw dataset formats, such as, JASON, CSV. Hence, \sysname{} enables groundbreaking methodologies and innovative approaches to accelerate the process of building data science applications. This Section presents our on-demand automation for predicting a data cleaning or transformation operation and selecting a classifier with its near-optimal parameters (AutoML) while developing a pipeline for datasets that have never been used for building the LiDS graph (a.k.a unseen dataset). 

Our on-demand automation is based on GNN models trained to predict a near-optimal operation/classifier for an unseen dataset $d_u$ based on the set of operations/classifiers used with similar (seen) dataset $d_s$ in our KG, LiDS. More specifically, we measure the cosine similarity between the embeddings of $d_u$ and $d_s$ to do what?????. Note that each $d_u$ is associated with a modelling task, such as predicting survivals in the Titanic dataset shown in Figure 3. The objective of this on-demand automation is to clean, prepare the dataset and choose the model parameter to maximize the model performance for the associated task. This is different, in principle, from existing data cleaning systems that perform general cleaning to recover the original data.

\input{tables/cleaning_transformation_operations}

\subsection{Training and Inference}

%\sysname{} could be queried to fetch the cleaning or transformation operations and dataset nodes of type columns or tables used as input. For instance, the training dataset could include frequently used transformation operations to train data transformation recommendation models. Such cases can be observed in figure \ref{fig:kglids_visualization}, where the operation StandardScaler is applied to the column 'Age'. Then, 
We train all GNN models on the LiDS graph. We use CoLR embeddings to initialize the embeddings of dataset nodes, i.e., nodes of type columns or tables. Table embeddings are calculated by averaging column embeddings, grouped by their data type. The length of each embedding is $300$, and since there are 6 fine-grained data types\footnote{The $7^{th}$ data type in our system is Boolean, but it does not have an embedding.}, the total length of all embeddings concatenated is $1,800$. These models only have one layer because there is only one edge between a given table and its potential operations. 

In this paper, we trained \sysname{}'s models using the top-rated $1000$ Kaggle datasets and associated $13,800$ pipeline scripts with the highest number of votes. Table~\ref{table:cleaning_trans_operations} highlights examples of cleaning and transformation operations collected from our Kaggle KG. We utilized GraphSAINT~\cite{GraphSAINT} to train GNN models for our node classification models for predicting operations for data cleaning and transformation.   



In the inference phase, a GNN model takes the unseen dataset in the form of a DataFrame and calculates the CoLR embedding for each column. It then leverages a task-specific pre-trained model to predict the most relevant operation to apply on the dataset. %Our GNN models are based on fixed-size embeddings that enable concise summarization of a dataset of large content. Hence, our on-demand automation excels in scalability for providing data preparation recommendations. 







\subsection{Data Cleaning}
\label{subsec:data_cleaning}

We formalize the task of data cleaning recommendation as a multiclass node classification problem. Given a dataset $\mathcal{D}$ with missing values $\mathcal{M}=\{m_1,m_2,...,m_n\}$ and a machine learning task $\mathcal{L}$, the recommendation task is to predict the cleaning operation $c_r \in \mathcal{C}$ to handle $\mathcal{M}$ such that the accuracy of $\mathcal{L}$ is improved based on the cleaning techniques applied by other data scientists in other datasets similar to $\mathcal{D}$. 
% As part of its data cleaning, \sysname{} also performs outlier detection and repairs it by framing the outlier detection as a binary classification problem where for the same dataset $\mathcal{D}$, \sysname{} can detect whether outliers exist in the dataset.
For data cleaning, the output of the model can be one of 5 cleaning operations (Fillna, Interpolate, SimpleImputer, KNNImputer, IterativeImputer). 


\sysname{} provides several task-specific APIs such as:\shorten
\begin{Verbatim}[commandchars=\\\{\}]
{\small
\textbf{{\color{blue}cleaning_info}} = \textbf{recommend_cleaning_operations(}df\textbf{)}
}
\end{Verbatim}
that provide data cleaning recommendations. Additionally, \sysname{} provides another set of APIs that enable data scientists to directly select and apply the recommended data cleaning operations to their dataset without requiring explicit code. For instance, the following API:\shorten
\begin{Verbatim}[commandchars=\\\{\}]
{\small
\textbf{clean(}df, \textbf{{\color{blue}cleaning_info.iloc[0]})}
}
\end{Verbatim}
takes the base dataframe and selected cleaning operation as input and returns the cleaned dataset as output. %\sysname{} has similar APIs to support data transformation and modelling.  


\subsection{Data Transformation}
\label{subsec:data_transformation}

Similar to data cleaning, we formalize the task of data transformation recommendation as a node classification problem. Given a dataset $\mathcal{D}$ with features $\mathcal{F}=\{f_1,f_2,...,f_n\}$ and a machine learning task $\mathcal{L}$, the recommendation task is to predict a set of transformations $\mathcal{T}=\{t_1,t_2,...,t_m\}$ to improve the accuracy of $\mathcal{L}$ based on the transformation techniques applied by other data scientists in the past on datasets and features similar to $\mathcal{D}$ and $\mathcal{F}$ respectively. The problem of data transformation recommendation is subdivided into two primary steps: 1) recommending Table transformations (Standard Scaler, Minmax Scaler, and Robust Scaler) first to avoid challenges of varying data magnitudes \cite{scaling_helps}; and then 2) recommending column transformations (log and sqrt). %It was noticed that not all columns required a unary transformation, and therefore, the option of not applying any transformations was added to the model.
Each transformation has its own training dataset and GNN model. \shorten




%\subsection{Data Cleaning}
%\label{subsec:data_cleaning}

%We formalize the task of data cleaning recommendation as a multiclass node classification problem. Given a dataset $\mathcal{D}$ with missing values $\mathcal{M}=\{m_1,m_2,...,m_n\}$ and a machine learning task $\mathcal{L}$, the recommendation task is to predict a cleaning operation $c_r \in \mathcal{C}$ to handle $\mathcal{M}$ such that the accuracy of $\mathcal{L}$ is improved based on the cleaning techniques applied by other data scientists in other datasets similar to $\mathcal{D}$. 
% As part of its data cleaning, \sysname{} also performs outlier detection and repairs it by framing the outlier detection as a binary classification problem where for the same dataset $\mathcal{D}$, \sysname{} can detect whether outliers exist in the dataset.

%Our GNN model is initialized using table embeddings, which are derived from our column embeddings. These embeddings are calculated by averaging the embeddings of the columns in the table that contain missing values. Separate averages are computed for each column datatype, and these averaged embeddings are then concatenated. As our embeddings are of length 300, the embeddings used to initialize the GNN model are of length 1800. Given that the output of the model can be one of 5 cleaning operations (Fillna, Interpolate, SimpleImputer, KNNImputer, IterativeImputer), our GNN model will have 1800 input channels and five output channels. The GNN model will only have one layer as there is only one edge between a given table and its cleaning operation. The trained model is capable of predicting the node associated with a given table in the context of cleaning operations.

%\subsection{Data Transformation}
%\label{subsec:data_transformation}
%We formalize the task of data transformation recommendation as a node classification problem. Given a dataset $\mathcal{D}$ with features $\mathcal{F}=\{f_1,f_2,...,f_n\}$ and a machine learning task $\mathcal{L}$, the recommendation task is to predict a set of transformations $\mathcal{T}=\{t_1,t_2,...,t_m\}$ to improve the accuracy of $\mathcal{L}$ based on the transformation techniques applied by other data scientists in the past on datasets and features similar to $\mathcal{D}$ and $\mathcal{F}$ respectively. The problem of data transformation recommendation is subdivided into two primary steps: 1) recommending Table transformations (Standard Scaler, Minmax Scaler, and Robust Scaler) first to avoid challenges of varying data magnitudes \cite{scaling_helps}; and then 2) recommending column transformations (log and sqrt). Each transformation has its own training dataset and GNN model. 
%The primary motivation behind employing scaling transformations prior to unary transformations lies in addressing the challenges of varying data magnitudes \cite{scaling_helps}. By scaling the data, we ensure that all features are treated on an equal footing, preventing certain features from overshadowing others due to their scale. \shorten
%We support two types of transformation: Table transformations (Standard Scaler, Minmax Scaler, and Robust Scaler) and column transformations (log and sqrt). 
%Each transformation has its own training dataset and GNN model. %Our training dataset contains triples similar to those used for the cleaning model, with only the predicate $<$hasCleaningOperation$>$ now replaced by $<$hasScalingTransformation$>$ and $<$hasUnaryTransformation$>$ respectively.
%
%The table transformation model is trained using averaged embeddings of each column type concatenated (1800) as initialization. The column transformation did not require any aggregation in its initialization as each column was directly associated with its embedding of size 300. It was noticed that not all columns required a unary transformation, and therefore, the option of not applying any transformations was added to the model.

\subsection{Our AutoML Support as a GNN Graph Generation Model}
The AutoML problem aims to select the near-optimal ML classifier with the set of parameters for a certain dataset. KGpip~\cite{kgpip} is the state-of-the-art AutoML system based on GNNs that have been trained on top of a data science KG. The initial version of KGpip was trained using a KG generated by a general-purpose code abstraction tool called GraphGen4Code\cite{graph4code}. Hence, the offline training phase of KGpip involves extensive graph filtration to remove noisy nodes that are not relevant to data science artifacts, as stated in~\cite{kgpip}. The inference phase includes using the KGpip model to predict a classifier. Then, KGpip utilizes a hyperparameter optimizer to search for near-optimal set of parameters for the predicted classifier.   


{\sysname} improves KGpip system in two ways. First, the {\graphname} graph maintains only the semantics of data science artifacts. Hence, {\sysname} helps KGpip avoid the extensive graph filtration step. Second and more importantly, unlike GraphGen4Code, the {\graphname} augments all function calls with the parameter names used by analyzing the relevant programming documentation. Hence, the {\graphname} includes for each classifier the set of pairs (parameter name and value) used for each function call. 
These values improved the KGpip inference pipeline because they are used 
as an initial configuration for the hyperparameter search on unseen datasets. This initialization significantly reduced the search time and improved the accuracy of the KGpip AutoML system. 


==> sections/dataPreparation.tex <==
% \subsection{GNN-based Data Preparation Models}
\subsection{On-demand Data Preparation based on GNN Models}
\label{sec:dPrep}


\subsubsection{Data Cleaning}
\label{subsec:data_cleaning}

We formalize the task of data cleaning recommendation as a multiclass classification problem. Given a dataset $\mathcal{D}$ with missing values $\mathcal{M}=\{m_1,m_2,...,m_n\}$ and a machine learning task $\mathcal{L}$, the recommendation task is to predict the cleaning operation $c_r \in \mathcal{C}$ to handle $\mathcal{M}$ such that the accuracy of $\mathcal{L}$ is improved based on the cleaning techniques applied by other data scientists in other datasets similar to $\mathcal{D}$. 
As part of its data cleaning, \sysname{} also performs outlier detection and repairs it by framing the outlier detection as a binary classification problem where for the same dataset $\mathcal{D}$, \sysname{} can detect whether outliers exist in the dataset.

\input{tables/cleaning_transformation_operations}

\emph{Training.} Both a cleaning classification model and an outlier detection model are trained for data cleaning. To build the cleaning classification model, the \graphname{} graph is queried to fetch the datasets with missing values and the applied data cleaning operations. These operations include the most frequently used data cleaning operations.%, such as \emph{Fill}, \emph{Imputation}, and \emph{Interpolation}. 
 Next, the CoLR embeddings for the dataset are generated. 
% This generates the  modeling data for data cleaning where feature embeddings represent the independent variables and the data cleaning operation represents the corresponding target.
%
Finally, we train a deep neural network model to recommend data cleaning operations on three classes, including \emph{Fill}, \emph{Imputation}, and \emph{Interpolation}. The outlier detection model is built similarly, with the \graphname{} graph being queried for datasets on which outlier detection is applied. To build a balanced classification model, datasets on which outlier detection is not applied are added to the training set. The average of the CoLR embeddings for all datasets in the training set is computed. We trained a Random Forest Classifier to determine whether there was a need for outlier detection. 



\subsubsection{Data Transformation}
\label{subsec:data_transformation}
We formalize the task of data transformation recommendation as a classification problem. Given a dataset $\mathcal{D}$ with features $\mathcal{F}=\{f_1,f_2,...,f_n\}$ and a machine learning task $\mathcal{L}$, the recommendation task is to predict a set of transformations $\mathcal{T}=\{t_1,t_2,...,t_m\}$ to improve the accuracy of $\mathcal{L}$ based on the transformation techniques applied by other data scientists in the past on datasets and features similar to $\mathcal{D}$ and $\mathcal{F}$ respectively. The problem of data transformation recommendation is subdivided into two primary steps: 1) recommending scaling transformations (applied to the entire dataset) and 2) recommending unary feature transformations (applied to an individual feature of the dataset). The primary motivation behind employing scaling transformations prior to unary transformations lies in addressing the challenges of varying data magnitudes \cite{scaling_helps}. By scaling the data, we ensure that all features are treated on an equal footing, preventing certain features from overshadowing others due to their scale. \shorten

\emph{Training.} The \graphname{} graph is queried to fetch the features and the applied data transformation operations. These operations comprise all scaling transformations provided in the \emph{Scikit-learn} library: \emph{StandardScaler}, \emph{MinMaxScaler}, \emph{RobustScaler} and \emph{MaxAbsScaler} and the most used unary feature transformation techniques that are provided in the \emph{NumPy} and \emph{Scikit-learn} library: \emph{Log}, \emph{Sqrt}, \emph{Square}, \emph{Tanh}, \emph{OrdinalEncoder} and \emph{OneHotEncoder}. %Unary transformations are valuable for manipulating data in machine learning \cite{lfe}.% However, to maximize their effectiveness, applying scaling transformation beforehand can improve the performance of unary transformations, leading to improved model effectiveness.  %For instance, algorithms like KNN and SVM rely on measuring the distance between data points. 
% Without proper scaling, features with larger values tend to dominate the feature similarity measurement, leading to suboptimal or inadequate model performance \cite{scaling_helps}. 
% By scaling the data, we ensure that all features are treated on an equal footing, preventing certain features from overshadowing others due to their inherent scale.%, thus facilitating a balanced and unbiased unary transformation.% Another compelling reason for utilizing scaling transformation is its efficacy in handling outliers. Outliers, characterized by extreme values, can significantly impact unary transformations by causing distortion in the transformation process and hindering accurate modeling. By scaling the data, we effectively reduce the influence of outliers, enabling the unary transformations to exhibit greater robustness and resilience. Thus incorporating scaling transformations before unary transformations offers a range of benefits that positively impact the performance.
The transformed features obtained from the graph are then associated with their respective CoLR embeddings. Scaling transformations are performed on the entire dataset, ensuring that all features are appropriately scaled. Subsequently, the embeddings for all transformed features within a dataset are averaged to create a comprehensive representation of the dataset. However, in the case of unary transformations, the embeddings remain unchanged, capturing the characteristics of the individual transformed feature. Finally, we train an independent deep neural network classifier per transformation type and feature type: %, i.e., one classification model to recommend the scaling data transformation and two separate classification models to recommend unary data transformation for numerical and categorical features, respectively. Thus, in the modeled data for data transformation, the feature embeddings represent the independent variables, and the data transformation technique represents the corresponding target. We train a deep neural network to recommend data transformation per transformation type and feature type. This includes: 
1. Scaling transformation model trained on four classes: \emph{StandardScaler}, \emph{MinMaxScaler}, \emph{RobustScaler} and \emph{MaxAbsScaler} making it a multiclass classification problem. 2. Numerical Unary transformation model trained on six classes: \emph{Log}, \emph{Sqrt}, \emph{Square}, \emph{Tanh}, \emph{OrdinalEncoder} and \emph{OneHotEncoder}. 3. Cateogrical transformation model trained on two classes \emph{OrdinalEncoder} and \emph{OneHotEncoder} making it a binary classification problem.\shorten% For all these three models the feature embeddings represent the independent variables, and the data transformation technique represents the corresponding target. \shorten





==> sections/dataPreparation_nm.tex <==
% \subsection{GNN-based Data Preparation Models}
\subsection{On-demand Data Preparation based on GNN Models}
\label{sec:dPrep}


\subsubsection{Data Cleaning}
\label{subsec:data_cleaning}
\subsubsubsection{Description of the graph used for training:}
1014 datasets and their 20 most popular notebooks were profiled using kglids. From this data, the datasets containing missing values were selected. The resulting graph will have nodes such as table, column, path, as well as edges such as hasContentSimilarity, hasMissingValueCount, and isPartOf from the actual dataset and the nodes Value, SimpleImputer, KNNImputer and Fillna as well as the edges HasCleaningOperation, SimpleImputer, KNNImputer, IterativeImputer, Interpolate and Fillna which come from profiling the notebooks related to the datasets. Different notbooks might use different cleaning operations on the same table. To express that, two types of triples are used to express the cleaning operations used on a table. An example triple would be $<$Table$>$$<$HasCleaningOperation$>$$<$Fillna$>$ or $<$Table$>$$<$Fillna$>$$<$Value$>$, where the first triple dictates that the cleaning operation Fillna is the most commonly used operation on a given table while the second triple shows the number of notebooks that used the Fillna operation for the given table.


\input{tables/cleaning_transformation_operations}


\subsubsubsection{Training}
In the training phase, the kglids graph is encoded, with the target relation being $<$HasCleaningOperation$>$ and the label node designated as $<$Table$>$. A Relational Graph Convolution Network (RGCN) is employed to build a model that will predict the node associated with the edge $<$HasCleaningOperation$>$ for a given table node.

The RGCN model is initialized using table embeddings, which are derived from kglids' column embeddings. These embeddings are calculated by averaging the embeddings of the columns in the table that contain missing values. Separate averages are computed for each column datatype and these averaged embeddings are then concatenated together. As kglids' embeddings are of length 300, the embeddings used to initialize the RGCN model are of length 1800. Given that the output of the model can be one of 5 cleaning operations (Fillna, Interpolate, SimpleImputer, KNNImputer, IterativeImputer), our RGCN will have 1800 input channels and 5 output channels. The RGCN model will only have one layer as there is only one edge between a given table and its cleaning operation.
The resulting model is capable of predicting the node associated with a given table in the context of cleaning operations.

\subsubsubsection{Inference:}
During the inference phase, an unseen dataset to be tested is transformed into a graph representation consisting of nodes $<$Table$>$ and $<$Column$>$, connected by the $<$isPartOf$>$ edge type. This graph is then encoded.

The RGCN model, which has been pre-trained, is loaded for inference. Since the dataset typically contains only one table in this context, the embedding for that single table is calculated following the earlier process. This embedding is used to initialize the RGCN model.

The RGCN model generates an output value ranging from 0 to 4. This output can be decoded to determine one of five possible cleaning operations that are most relevant to the given dataset, allowing for efficient and automated data cleaning decisions.

\subsubsection{Data Transformation}
\label{subsec:data_transformation}
\subsubsubsection{Description of the graph used for training:} From the 1014 datasets graphed, the datasets containing various transformations were selected as training data. Two types of transformation are done in this application: Table transformations (Standard Scaler, Minmax Scaler, and Robust Scaler) and column transformations (log and sqrt). Each has its own training dataset and model. Training graph built for each of these models contains triples similar to those used for the cleaning model, with only the predicate $<$hasCleaningOperation$>$ now replaced by $<$hasScalingTransformation$>$ and $<$hasUnaryTransformation$>$ respectively.

\subsubsubsection{Training:}
The table transformation model is built using averaged embeddings of each column type concatenated (1800) as initialization, resulting in an input of 1800 and output of 3 as the output results are Standard Scaler, Minmax Scaler, and Robust Scaler.
The column transformation did not require any aggregation in its initialization as each column was directly associated to its embedding of size 300. It was noticed that not all columns required a unary transformation and therefore the option of not applying any transformations was added to the model, resulting in an input of 300 and output of 3 the output results are log, sqrt, and none.

\subsubsubsection{Inference:}
The inference phase is similar to that of data cleaning, with the difference that in addition to the transformation prediction for the entire table, column transformations are also recommended for each individual column. The Scaling operation is first applied on the entire table before applying the unary transformations on each column separatly. 



==> sections/evalDataPrep-Don_tUSE.tex <==
\subsection{Evaluating Our On-Demand Automation Models}
\label{sec:evaluationDataPrep}

\subsubsection{Data Cleaning} 
In this set of experiments, we used the eight datasets from the AutoML benchmarks~\cite{kgpip} that contained missing values and supplemented them with five datasets from the UCI repository \cite{uci}. Our evaluation consisted of cleaning these datasets using \sysname{} and \holoclean{}. Our evaluation metric includes the F1 scores of a random forest classifier trained using cross-validation over ten folds on the cleaned datasets. 



\input{tables/cleaning_results}

\input{tables/transformation_results}

In Figure \ref{fig:exp_data_cleaning}, it can be observed that \sysname{} has a consistently high F1 scores. Regarding efficiency, \sysname{} is outperforming HoloClean in 85\% of datasets concerning time and in 38\%  datasets w.t.o the memory usage respectively. However, it can be obsereved that the disadvantage in memory usage is erased as the datasets get larger as most of the memory used by \sysname{} is static.
%
\holoclean{} faced memory constraints while attempting to clean datasets 11, 12, and 13, resulting in an inability to complete the cleaning process for these datasets. These datasets are given an F1 score of 0 in Figure \ref{fig:exp_data_cleaning} (a) and marked with an 'x' on the x-axis in Figure \ref{fig:exp_data_cleaning} (b), indicating that no time values were obtained for these datasets and an 'x' on top of the bar in Figure \ref{fig:exp_data_cleaning} (c), indicating that the memory capacity of the machine used was exceeded. 

We also consider a baseline method that performs modeling without data cleaning. The baseline method faced challenges with datasets, whose IDs are 2, 8, and 13. One notable advantage of \sysname{} is its ability to successfully complete the cleaning process on larger datasets, such as datasets whose IDs are 11, 12, and 13, where \holoclean{} encountered memory limitations. 
As a result, \sysname{} utilizes comparatively less memory compared to \holoclean{}, which generates multiple tables containing dataset information throughout its cleaning process. \sysname{} balances between efficiency and cleaning effectiveness, allowing users to clean their datasets effectively with little time and memory constraints.

\begin{figure}[t]
\vspace{-2ex}
  \centering
    \includegraphics[width=\columnwidth]{figures/cleaning_results_new_emb.png}
    \vspace*{-4ex}
    \caption{Data Cleaning: the performance of {\sysname} vs. Aimnet systems on multiple ML tasks on 13 datasets. 
    % (a) {\sysname{}} is the only system capable of completing the task on all datasets and outperforms both the baseline and \holoclean{} in 7 out of the 13 datasets (b) and (c) the time and memory consumed per system to perform data cleaning on the dataset and train the model. 
    Aimnet exceeds the memory budget in several cases. {\sysname} outperforms in most cases Aimnet in terms of accuracy while consuming  less time and almost a fixed amount of memory.} 
  \label{fig:exp_data_cleaning}
  \vspace{-2ex}
\end{figure}

\begin{figure}[t]
% \vspace{-2ex}
\centering
\includegraphics[width=\columnwidth]{figures/transformation_autolearn.png} 
\vspace*{-4ex}
  \caption{Data Transformation: the performance of {\sysname} vs. \autolearn{} on multiple ML tasks using 18 datasets. (a) and (b) the time and memory consumed per system to perform data transformation on the dataset. {\sysname} outperforms \autolearn{} in terms of time while memory usage does not significantly increase with large datasets.}
  \label{fig:transformation_autolearn}
  \vspace*{-2ex}
\end{figure}

\subsubsection{Data Transformation} This set of experiments compared \sysname{} to \autolearn{} using the datasets from \autolearn{}'s experimental evaluation \cite{autolearn} available in the UCI repository \cite{uci}. Our evaluation procedure involved applying the data transformation recommended by \sysname{} and \autolearn{} to each dataset. Subsequently, we trained a random forest classifier using a 5-fold cross-validation approach. 
Table~\ref{tab:transformation_results} shows the accuracy achieved by each system. We illustrate the full time and memory consumed by each system in Figure~\ref{fig:transformation_autolearn}.(a) and (b), respectively.  \sysname{} outperformed \autolearn{} on 65\% of the datasets in the accuracy metric while consuming less time and almost fixed memory w.r.t \autolearn{}. 










\begin{figure}[t]
% \vspace*{-2ex}
 \centering
  \includegraphics[width=\columnwidth]{figures/automl_results_vs_graph4_code.pdf} 
  \vspace*{-3ex}
  \caption{F1-Score difference between KGpip with GraphGen4Code and KGpip with KGLiDS on 24 binary and multi-class classification AutoML datasets, where the difference between both systems is $> 0.01$.}
  \label{fig:automl_experiment}
  \vspace*{-2ex}
\end{figure}

\subsubsection{AutoML}

We integrated the revised version of the KGpip pipeline into {\sysname}. The inference pipeline utilizes {\graphname} to recommend a starting point for the hyperparameter search. The recommended initial hyperparameters by {\sysname} for a given dataset are the most commonly used for the top-voted pipelines associated with the most similar dataset found in the {\graphname} graph. 
Figure \ref{fig:automl_experiment} shows a comparison in the F-Score of the original KGpip pipeline ($Pip_{G4C}$) using GraphGen4Code and our revised pipeline ($Pip_{LiDS}$) using our {\graphname} graph. We follow the same evaluation procedure in~\cite{kgpip} and limit the time budget to 40 seconds to avoid the exploration of the full search space. 
$Pip_{LiDS}$ outperforms $Pip_{G4C}$ in the majority of datasets, with an absolute difference in F-Score reaching 0.29 in some datasets. In addition, a \textit{two-tailed t-Test} between the scores obtained from both pipelines shows that $Pip_{LiDS}$ has significantly better scores with a t-Test value of $0.012$ ($p < 0.05$). This shows that by using the {\graphname} graph, an AutoML system can directly benefit from the accumulated knowledge of data scientists to improve the score or reduce the time budget required for exploring the hyperparameter search space.\shorten




% We evaluated the usability of {\sysname} for the problem of automatically generating optimized ML pipelines (AutoML). As described in Section \ref{sec:automl_use_case}, we integrated {\sysname} within KGpip, an AutoML framework that utilizes GraphGen4Code and graph neural networks to generate ML pipelines. We used {\sysname} to generate pipeline graphs for the same training set of KGpip. % This recommendation is formulated as a SPARQL query that executes within 361 milliseconds on average. GraphGen4Code does not maintain information on dataset similarities or pipeline votes and, therefore, cannot provide such a recommendation. 
%

==> sections/evaluation-essam-nov28.tex <==
%!TEX root = ../paper.tex

\section{Experimental Evaluation}
\label{sec:evaluation}


There is no other holistic system in the literature that combines the semantics of code (data science pipelines) and data. Therefore, it is not possible to evaluate {\sysname}'s performance with any single system. Instead, we evaluate {\sysname} against state-of-the-art (SOTA) systems in four real-world applications, namely, table union search, data cleaning, data transformation, and automated machine learning (AutoML). For all compared systems, we used the same configurations and hyper-parameters recommended by their authors. Our evaluation shows that {\sysname} can achieve competitive accuracy compared to these SOTA systems, which are specifically designed for each task. Furthermore, {\sysname} shows superior efficiency in terms of time and memory.

\input{tables/data_discovery_dataset_stats}

\nsstitle{Experiment Setup}
We used GraphDB\footnote{\url{https://www.ontotext.com/products/graphdb/}} version \textit{10.4.1} as an RDF engine to store the {\graphname} graph. 
% We deployed the endpoint, {\sysname}, and GrapGen4Code on the same local machine. 
We used two different hardware settings for our experiments. For data cleaning, data transformation, and AutoML experiments, we used Ubuntu 22.04, a 16-core CPU at 2.40 GHz, and 189 GB of RAM. For data discovery experiments, we used Ubuntu 22.04, a 64-core CPU at 2.45 GHz, 1TB of RAM, and an Nvidia A100 GPU.\shorten


% For systems evaluation, we used a total of {\totalDatasets} \textbf{unseen} datasets, collected from different benchmarks. A complete list of the {\totalDatasets} datasets including their ID and statistics is available at our {\sysname} repository\footnote{\url{https://github.com/CoDS-GCS/kglids/tree/master/gnn_applications}}. Each dataset is associated with an ML task. For example, we perform data preparation or feature engineering using one of the systems and then model the task. We consider the model utility score as our primary metric to measure the accuracy of each system. \shorten



\subsection{{\sysname} vs Data Discovery Systems}

We evaluate {\sysname} against two SOTA systems that achieve the highest scores in recent benchmarks: Starmie~\cite{starmie} and SANTOS~\cite{santos}. Stramie discovers unionable tables via column embeddings from pre-trained language models, while SANTOS uses open and synthesized knowledge bases to match column relationships within tables. As defined in \cite{d3l, Fatemeh18, santos}, table unionability for a query table $T$ is calculated in terms of Precision$@k$ and Recall$@k$ for different values of $k$, such that $k$ is the number of desired unionable tables to $T$. The precision and recall are calculated for each $k$ as the averages over $N$ query tables.  
%
We evaluate the effectiveness using three benchmarks: 
\texttt{$D^3L$ Small}\footnote{\url{https://github.com/alex-bogatu/DataSpiders}}~\cite{d3l}, 
\texttt{TUS Small}\footnote{\url{https://github.com/RJMillerLab/table-union-search-benchmark}}~\cite{Fatemeh18}, and 
\texttt{SANTOS Small}~\cite{santos} \footnote{\url{https://github.com/northeastern-datalab/santos}}. 
\texttt{$D^3L$ Small} is a collection of $654$ real-world tables, where each table in the lake is manually annotated with all other related tables. \texttt{TUS Small} and \texttt{SANTOS Small} are collections of $1,539$ and $550$ synthetic tables, respectively, generated using random horizontal and vertical partitioning from real-world tables.\shorten 

Note that the \texttt{$D^3L$ Small} is the most challenging because it was manually annotated rather than synthetically generated, has the highest number of rows per table on average, and has a high number of unionable tables of 110 on average. %Therefore, we follow \cite{santos} and evaluate unionability on \texttt{SANTOS Small} only up to $k = 10$. 
Furthermore, because SANTOS requires additional manual annotation of intent columns for all tables, we followed the authors' recommendation of using the first columns as intent columns for \texttt{$D^3L$ Small}.
%
In addition, we evaluated {\sysname}'s scalability using \texttt{SANTOS Large}~\cite{santos}, which contains $11,090$ tables without ground truth. The statistics of these benchmarks are shown in Table \ref{tab:data_discovery_dataset_stats}.
%
In our evaluation, we used the same values of $(N,k)$ as in previous evaluations. More specifically, for \texttt{$D^3L$ Small} we used $(50, 185)$, for \texttt{TUS Small} we used $(150, 60)$, and for \texttt{SANTOS Small} we used $(50, 10)$.\shorten


\input{tables/scalability}

Figure \ref{fig:experiment_precision_recall} shows the average Precision@k and Recall@k for the different systems and benchmarks.
{\sysname} significantly outperforms Starmie and SANTOS in terms of precision and recall on $D^3L$ \texttt{Small} and \texttt{TUS Small}.
This outstanding performance shows the advantage of our CoLR models, which are designed and trained per fine-grained data type. 
% $D^3L$ uses hand-crafted feature vectors, which do not capture all aspects of the columns.
Unlike {\sysname}, Starmie uses column embeddings from pre-trained language models, which work well with textual columns but do not achieve the same accuracy for numerical columns. We analyzed Starmie's individual column matches for $D^3L$ \texttt{Small}, which had 52.2 precision for numerical columns compared to 63.4 for textual columns. In addition, our CoLR models are trained to predict column similarity even with different value distributions, which enhances similarity prediction for real-world benchmarks like $D^3L$ \texttt{Small}. 
{\sysname} still achieves high accuracy for synthetically generated benchmarks, where unionable tables have the same distribution.
Finally, breaking down similarity prediction in the data lake into 7 smaller fine-grained tasks, one per column data type (Table \ref{tab:data_discovery_dataset_stats}), helps greatly reduce the false-positives of {\sysname}. 
%
For the \texttt{Santos Small} benchmark, the difference between the systems is less pronounced due to the small value of $k$ (as per the ground truth provided by the authors). Nonetheless, {\sysname} maintains a consistently high precision and recall for all values of $k$. For recall, {\sysname} consistently achieves comparable recall to Starmie and SANTOS. 

\begin{figure}
\vspace*{-2ex}
 \centering
\includegraphics[width=\columnwidth]{figures/smaller_real_and_santos_and_tus_precision_recall_column.pdf} 
\vspace*{-4ex}
  \caption{Average precision and recall of unionable table discovery on all benchmark datasets.}
\label{fig:experiment_precision_recall}  
\vspace*{-3ex}
\end{figure}

\subsubsection{Performance and Scalability Analysis} 
This experiment analyzes the system performance of {\sysname}, Starmie, and SANTOS. For fairness, this analysis is conducted on a single machine because SANTOS and Starmie do not support running on a cluster of machines. We focused on the preprocessing time, i.e., the offline time required to analyze the tables in a data lake, and the average query time, i.e., the time required to retrieve unionable tables given a query table, averaged over all query tables (see Table \ref{tab:data_discovery_dataset_stats} for the number of query tables for each benchmark).

Table~\ref{tab:scalability_vs_santos} summarizes our results. {\sysname} consistently outperforms SANTOS and Starmie in preprocessing and average query times for small and large benchmarks. We focus on the \texttt{SANTOS Large} benchmark as it has the largest number of tables.
{\sysname} is 7.3x faster than SANTOS in preprocessing time. This is because SANTOS analyzes data lake tables on the granularity of column values, matching each value against two knowledge bases (KB): an open KB (YAGO \cite{yago}) and a synthesized KB generated during preprocessing. SANTOS then iterates over \textit{all value pairs} of matching columns per table to determine their semantic relationships. {\sysname} analyzes data lakes on the granularity of columns and applies our CoLR models to column samples. 
Compared to Starmie, {\sysname} achieves a 1.8x speed up in preprocessing time. 
The preprocessing phase of Starmie includes training a language model (LM) to generate the column embeddings for a data lake. Starmie uses data augmentation on data lake columns to generate enough samples to train the LM. Further, Starmie needs to train the LM for enough number of epochs to achieve a decent score (we use 10 epochs as per the authors' recommendation). Unlike Starmie, {\sysname} does not require training the CoLR models per data lake to generate column embeddings because our models are independently pre-trained on Kaggle and OpenML datasets.\shorten 



Furthermore, {\sysname} is designed to scale for discovery queries by leveraging the built-in indices in RDF engines. Compared to SANTOS, {\sysname} is 51.2x faster on average for the \texttt{SANTOS Large} benchmark. For a query table, SANTOS retrieves a list of candidate unionable tables by looking up two indices (one for each KB) for column relationships similar to those found between pairs of columns in the query table. Then, the query table is matched against candidate tables at different granularities to determine the unionability score for each candidate. This results in a large number of comparison and higher query times for SANTOS. Similarly, {\sysname} is 3.3x faster than Starmie in average query time. While Starmie uses an efficient vector index (Hierarchical Navigable Small World (HNSW) \cite{hnsw}) to retrieve similar columns based on embeddings, it requires calculating an approximate distance between embeddings of size 768. However, a discovery query of {\sysname} takes a table graph node and utilizes efficient RDF indices to find unionable tables, which is significantly faster as shown in Table \ref{tab:scalability_vs_santos}. 
 



 
\subsubsection{Ablation Study of the {\sysname} Effectiveness}
This ablation study analyzes the effect of our embedding-based approaches. Figure \ref{fig:ablation_study} shows the precision and recall of different KGLiDS configurations on the \texttt{TUS Small} benchmark. The highest scores were achieved by utilizing both the CoLR and label embeddings (indicated by the green line). While column names are a strong predictor of table unionability for the shown benchmarks, raw value-based unionability is useful for data lakes without column names (e.g. anonymized). Figure \ref{fig:ablation_study} illustrates that KGLiDS still performs competitively when using only CoLR embeddings, i.e., predicting unionability based only on raw values (indicated as ``Fine-Grained").  

\begin{figure}[t]
\vspace*{-2ex}
\centering
\includegraphics[width=\columnwidth]{figures/unionability_ablation_study.pdf} 
\vspace*{-5ex}
  \caption{Ablation study for the effectiveness of {\sysname} for table union search on the \texttt{TUS Small} benchmark.}
  \label{fig:ablation_study}
  \vspace*{-2ex}
\end{figure}

% Furthermore, the impact of our approach to training CoLR models for seven fine-grained data types is shown. 
In comparison to the use of three coarse-grained embedding models as suggested by \cite{MuellerS19}, the fine-grained CoLR models yield significantly higher precision and recall, with precision reaching up to 17\% higher and recall up to 50\% higher at $k=60$. Finally, we evaluate the impact of subsampling columns when applying CoLR models as described in Section \ref{sec:data_profiling}. As shown, applying CoLR models on column samples of 10\% of the original column sizes performs comparably in both precision and recall to applying them on entire columns. However, our subsampling approach reduces the profiling time for the TUS Small benchmark by 14\%. Similar results to this ablation study are obtained on other benchmarks.







\subsection{{\sysname} and Pipeline Abstraction}
\label{sec:evaluation-pipelineGraphs}

We evaluate \sysname{} against GraphGen4Code~\cite{graph4code}. GraphGen4Code~\cite{graph4code} is a toolkit to generate a knowledge graph for code~\footnote{GrapGen4Code is obtained from \url{https://github.com/wala/graph4code}}. 
%
we collected $13,800$ data science pipeline scripts used in the top $1000$ datasets from Kaggle, which includes $3,775$ tables and $141,704$ columns \footnote{The script to download these datasets is available at {\sysname}' repository}. 
We selected these pipelines and datasets based on the number of users' votes on the Kaggle platform. For each dataset, we select up to 20 most voted Python pipelines. The datasets are related to various supervised and unsupervised tasks in different domains, such as health, economics, games, and product reviews.
%
Table \ref{tab:graph_analysis} summarizes the graph sizes and analysis times for generating the {\graphname} and GraphGen4Code graphs for the Kaggle pipelines dataset. For a fair comparison, we run the pipeline abstraction of {\sysname} on a single machine. Thanks to the lightweight static code, documentation, and dataset usage analyses employed by {\sysname}, it achieves a graph reduction of more than 82\% in 95\% less time for the same set of pipelines.\shorten



Furthermore, a breakdown of both graphs by the modelled aspects of data science pipelines is shown in Table \ref{tab:modelled_aspects}. Because the focus of GraphGen4Code is the abstraction of general-purpose code, it captures redundant information when used for data science pipelines.
For example, approximately 30\% of GraphGen4Code models local syntactical script information, namely, \emph{statement location}, \emph{variable names}, and \emph{function parameter order}. Without cleaning these aspects, two pipeline scripts with similar semantics could have dissimilar graphs in GraphGen4Code if e.g. they have different variable names. 
In contrast, {\sysname} captures semantics related primarily to data science, including ones not modelled by GraphGen4Code, such as \emph{dataset reads} that indicate when \texttt{CSV} files are read, or \emph{library hierarchy} that model the structure of functions and classes in a data science library. These aspects are essential for automating data science pipelines, such as discovering pipelines for similar datasets and highly effective libraries. In addition, all nodes in the {\graphname} graph are labeled with an RDF type, a standard requirement when constructing knowledge graphs for facilitating graph queries, building a graph schema, and enabling reasoning by RDF engines.


\input{tables/graph_anlaysis}
\input{tables/modelled_aspects}


\subsection{Evaluating Our On-Demand Automation Models}
\label{sec:evaluationDataPrep}
This section presents our evaluation for \sysname{} against SOTA systems in data cleaning, transfromation and AutoML. 
%
% For training our GNN models for data cleaning and transformation, we used the top-rated one thousand Kaggle datasets comprising $\sim$3.7k tables, $\sim$140k columns, and $\sim$13k pipelines to train \sysname{}'s data preparation recommendation models and control the quality of our recommendations. 
For systems evaluation, we used a total of {\totalDatasets} \textbf{unseen} datasets, collected from different benchmarks. A complete list of the {\totalDatasets} datasets including their ID and statistics is available at our {\sysname} repository\footnote{\url{https://github.com/CoDS-GCS/kglids/tree/master/gnn_applications}}. Each dataset is associated with an ML task. For example, we perform data preparation or feature engineering using one of the systems and then model the task. We consider the model utility score as our primary metric to measure the accuracy of each system. \shorten

\subsubsection{Data Cleaning} 
This experiment analyzes our on-demand cleaning against \holoclean{}, the SOTA general cleaning platform. \holoclean{} uses statistical learning and inference to unify a range of data-repairing methods. We used the most recent version of \holoclean{}, a.k.a Aimnet~\cite{aimnet}, where a user does not need to specify a set of denial constraints.   
We used the 13 datasets from an AutoML benchmark~\cite{kgpip} that contained missing values and supplemented them with five datasets from the UCI repository~\cite{uci}. Our evaluation process consisted of cleaning these datasets using \sysname{} and \holoclean{} and then training a random forest classifier. We also consider a baseline approach that performs modelling without any data cleaning. The evaluation metric we use to evaluate on-demand data cleaning includes the F1 scores of the random forest classifier trained using cross-validation over ten folds on the cleaned datasets. We also evaluate the cleaning systems in their efficiency in terms of execution time and memory requirements.\shorten

\input{tables/cleaning_results}

\input{tables/transformation_results}

Table~\ref{tab:cleaning_results} shows that our system (\sysname{}) has consistently higher F1 scores than \holoclean{}. Cleaning data using \holoclean{} led to a better performance in only one dataset, which had an F1 score above 95 for all systems anyway. 
%
Figure \ref{fig:exp_data_cleaning} shows that \sysname{} is outperforming \holoclean{} in $85\%$ of datasets in execution time and in $38\%$  datasets in memory usage. Note that the disadvantage of using more memory diminishes as the dataset gets larger because most of this memory is used by the training graph. %This also shows that \sysname{} can scale to very large datasets. 
For example, \holoclean{} failed with out-of-memory errors while attempting to clean datasets $\#11$, $\#12$, and $\#13$, and could not complete the cleaning process for these datasets. \holoclean{} generates multiple tables containing dataset information throughout its cleaning process. Therefore, its memory requirements increase as the dataset size increases. In contrast, \sysname{}'s memory requirement is almost constant because it relies on LiDS graph semantics. Hence, \holoclean{} is the right choice if the objective is to generally clean a dataset instead of improving the modelling performance while training a specific task on a dataset.\shorten 


\begin{figure}[t]
\vspace{-2ex}
  \centering
    \includegraphics[width=\columnwidth]{figures/cleaning_results_new_emb.png}
    \vspace*{-4ex}
    \caption{The performance of {\sysname} vs \holoclean{} (Aimnet) on the 13 datasets using a VM with 189 GB RAM. The X-axis represents the dataset ID, and the Y-axis is the time (a) or memory usage (b) consumed by each system. Datasets are sorted by size in increasing order. {\sysname} reduces the time significantly while using an almost fixed amount of memory across datasets, e.g., less than 4GB RAM.\shorten 
    } 
  \label{fig:exp_data_cleaning}
  \vspace{-2ex}
\end{figure}

\begin{figure}[t]
\vspace{-1ex}
\centering
\includegraphics[width=\columnwidth]{figures/transformation_autolearn.png} 
\vspace*{-4ex}
  \caption{
  The performance of {\sysname} vs \autolearn{} on the 18 datasets using a VM with 189 GB RAM. The X-axis represents the dataset ID, and the Y-axis is the time (a) or memory usage (b) consumed by each system. Datasets are sorted by size in increasing order. {\sysname} outperforms significantly \autolearn{} in terms of time, using an almost fixed amount of memory across datasets, e.g., less than 10GB RAM.\shorten}
  \label{fig:transformation_autolearn}
  \vspace*{-4ex}
\end{figure}



\subsubsection{Data Transformation} 

We compare \sysname{} against \autolearn{} \cite{autolearn}, a regression-based feature learning algorithm that automates feature engineering.
In this evaluation, we used datasets from~\autolearn{}'s experimental evaluation~\cite{autolearn}, which is available in the UCI repository~\cite{uci}. These datasets were assigned IDs from $14$ to $30$. 
Similar to data cleaning, our evaluation process includes applying the data transformation recommended by \sysname{} and \autolearn{} to each dataset and then we trained a random forest classifier.
%
The evaluation metric we use to evaluate on-demand data transformation includes the accuracy scores of the random forest classifier trained using cross-validation over 5-fold on the transformed datasets. We also evaluate the cleaning systems in their efficiency in terms of execution time and memory requirements. Table~\ref{tab:transformation_results} shows the accuracy achieved by each system. 


Figure~\ref{fig:transformation_autolearn} shows the execution time and memory usage of each system while transforming each dataset. X-axis is the dataset ID. Consistently with data cleaning results, \sysname{} outperformed its competitor in execution time, while memory usage did not increase dramatically as the data size increased. Overall, \sysname{} outperformed \autolearn{} on $65\%$ of the datasets in accuracy while consuming less time and almost fixed memory w.r.t \autolearn{}.  Autolearn's algorithm employs distance correlation to identify pairwise correlated features, classify them into linear and non-linear correlations, and then generate informative new features. These features are then ranked based on stability and information gain, with only the top ones selected. The original dataset's row and feature count, inter-feature correlations, created features, and the chosen feature quantity collectively impact Autolearn's memory usage. Hence, the dataset's absolute size is not the primary factor influencing memory usage in Autolearn's transformation.



\begin{figure}[t]
% \vspace*{-2ex}
 \centering
  \includegraphics[width=\columnwidth]{figures/automl_results_vs_graph4_code.pdf} 
  \vspace*{-3ex}
  \caption{ The F1-Score difference between KGpip with KGLiDS ($Pip_{LiDS}$) and KGpip with GraphGen4Code ($Pip_{G4C}$) across 24 AutoML datasets. The X-axis denotes the dataset IDs. 
  % The Y-axis is F1($Pip_{LiDS}$, ID) - F1($Pip_{G4C}$, ID).  
  $Pip_{LiDS}$ efficiently prunes hyperparameter search space and helps KGpip improve F1-Scores in most cases.
  }
  \label{fig:automl_experiment}
  \vspace*{-3ex}
\end{figure}


\subsubsection{AutoML and Better Hyperparameter Search}
We integrated the revised version of the KGpip pipeline into {\sysname}. The inference pipeline utilizes {\graphname} to recommend a starting point for the hyperparameter search. The recommended initial hyperparameters by {\sysname} for a given dataset are the most commonly used for the top-voted pipelines associated with the most similar dataset found in the {\graphname} graph. 
%
We used 24 benchmark tables used by the KGpip \cite{kgpip} system. The datasets pertain to different binary and multi-class classification tasks, are real-world datasets from a diversity of sources and problem domains, and are of enough difficulty for the learning algorithms.\shorten 


Figure \ref{fig:automl_experiment} shows a comparison in the F-Score of the original KGpip pipeline ($Pip_{G4C}$) using GraphGen4Code and our revised pipeline ($Pip_{LiDS}$) using our {\graphname} graph. We follow the same evaluation procedure in~\cite{kgpip} and limit the time budget to 40 seconds to avoid the exploration of the full search space. 
$Pip_{LiDS}$ outperforms $Pip_{G4C}$ in the majority of datasets, with an absolute difference in F-Score reaching 0.29 in some datasets. In addition, a \textit{two-tailed t-Test} between the scores obtained from both pipelines shows that $Pip_{LiDS}$ has significantly better scores with a t-Test value of $0.012$ ($p < 0.05$). This shows that by using the {\graphname} graph, an AutoML system can directly benefit from the accumulated knowledge of data scientists to improve the score or reduce the time budget required for exploring the hyperparameter search space.\shorten




==> sections/evaluation-old-khaled.tex <==
%!TEX root = ../paper.tex

\section{Experimental Evaluation}
\label{sec:evaluation}


There is no other holistic system in the literature that combines the semantics of code (data science pipelines) and data. Therefore, it is not possible to evaluate {\sysname}'s performance with any single system. Instead, we evaluate {\sysname} against state-of-the-art (SOTA) systems in four real-world applications, namely, table union search, data cleaning, data transformation, and automated machine learning (AutoML). For all compared systems, we used the same configurations and hyper-parameters recommended by their authors. Our evaluation shows that {\graphname} can achieve competitive accuracy compared to these SOTA systems, which are specifically designed for each task. Furthermore, {\sysname} shows superior efficiency in terms of time and memory.


\subsection{Experiment Setup}



We used GraphDB\footnote{\url{https://www.ontotext.com/products/graphdb/}} version \textit{10.4.1} as an RDF engine to store the {\graphname} graph. 
% We deployed the endpoint, {\sysname}, and GrapGen4Code on the same local machine. 
We used two different hardware settings for our experiments. For data cleaning, data transformation, and AutoML experiments, we used Ubuntu 22.04, a 16-core CPU at 2.40 GHz, and 567 GB of RAM. For data discovery experiments, we used Ubuntu 22.04, a 64-core CPU at 2.45 GHz, 1TB of RAM, and an Nvidia A100 GPU.


For systems evaluation, we used a total of {\totalDatasets} \textbf{unseen} datasets, collected from different benchmarks. A complete list of the {\totalDatasets} datasets including their ID and statistics is available at our {\sysname} repository\footnote{\url{https://github.com/CoDS-GCS/kglids/tree/master/gnn_applications}}. Each dataset is associated with an ML task. For example, we perform data preparation or feature engineering using one of the systems and then model the task. We consider the model utility score as our primary metric to measure the accuracy of each system. \shorten



\subsection{{\sysname} vs Data Discovery Systems}

In an extensive collection of datasets, such as a data lake, one of the data discovery tasks is to find unionable tables. As defined in \cite{d3l, Fatemeh18, santos}, table unionability for a certain table $T$ is calculated in terms of Precision$@k$ and Recall$@k$ for different values of $k$, such that $k$ is the number of desired unionable tables to $T$. The precision and recall are calculated as the averages over $N$ query tables sampled at random.  

We evaluate {\sysname} against two SOTA systems that achieve the highest scores in recent benchmarks: Starmie~\cite{starmie} and SANTOS~\cite{santos}. Stramie discovers unionable tables via column embeddings from pre-trained language models, while SANTOS uses open and synthesized knowledge bases to match column relationships within tables. 

We evaluate the effectiveness using three benchmarks: 
\texttt{$D^3L$ Small}\footnote{\url{https://github.com/alex-bogatu/DataSpiders}}~\cite{d3l}, 
\texttt{TUS Small}\footnote{\url{https://github.com/RJMillerLab/table-union-search-benchmark}}~\cite{Fatemeh18}, and 
\texttt{SANTOS Small}~\cite{santos} \footnote{\url{https://github.com/northeastern-datalab/santos}}. 
\texttt{$D^3L$ Small} is a collection of $654$ real-world tables, where each table in the lake is manually annotated with all other related tables. \texttt{TUS Small} and \texttt{SANTOS Small} are collections of $1,539$ and $550$ synthetic tables, respectively, generated using random horizontal and vertical partitioning from real-world tables. 

Note that the \texttt{$D^3L$ Small} is the most challenging because it was manually annotated rather than synthetically generated, has the highest number of rows per table on average, and has a high number of unionable tables of 110 on average. %Therefore, we follow \cite{santos} and evaluate unionability on \texttt{SANTOS Small} only up to $k = 10$. 
Furthermore, because SANTOS requires additional manual annotation of intent columns for all tables, we followed the authors' recommendation of using the first columns as intent columns for \texttt{$D^3L$ Small}.

In addition, we evaluated {\sysname}'s scalability using \texttt{SANTOS Large}~\cite{santos}, which contains $11,090$ tables without ground truth. The statistics of these benchmarks are shown in Table \ref{tab:data_discovery_dataset_stats}.


In our evaluation, we used the same values of $(N,k)$ as in previous evaluations. More specifically, for \texttt{$D^3L$ Small} we used $(100, 185)$, for \texttt{TUS Small} we used $(150, 60)$, and for \texttt{SANTOS Small} we used $(50, 10)$.


\input{tables/data_discovery_dataset_stats}



Figure \ref{fig:experiment_precision_recall} shows the average Precision@k and Recall@k for the different systems and benchmarks.
{\sysname} significantly outperforms Starmie and SANTOS in terms of precision and recall on $D^3L$ \texttt{Small} and \texttt{TUS Small}.
This outstanding performance shows the advantage of our CoLR models, which are designed and trained per fine-grained data type. 
% $D^3L$ uses hand-crafted feature vectors, which do not capture all aspects of the columns.
Unlike {\sysname}, Starmie uses column embeddings from pre-trained language models, which work well with textual columns but do not achieve the same accuracy for numerical columns. We analyzed Starmie's individual column matches for $D^3L$ \texttt{Small}, which had 52.2 precision for numerical columns compared to 63.4 for textual columns. In addition, our CoLR models are trained to predict column similarity even with different value distributions, which enhances similarity prediction for real-world benchmarks like $D^3L$ \texttt{Small}. Finally, breaking down similarity prediction in the data lake into 7 smaller fine-grained tasks, one per column data type (Table \ref{tab:data_discovery_dataset_stats}), helps greatly reduce the false-positives of {\sysname}. 

\begin{figure}
\vspace*{-2ex}
 \centering
\includegraphics[width=\columnwidth]{figures/smaller_real_and_santos_and_tus_precision_recall_column.pdf} 
\vspace*{-4ex}
  \caption{Average precision and recall of unionable table discovery on all benchmark datasets.}
\label{fig:experiment_precision_recall}  
\vspace*{-2ex}
\end{figure}


For the \texttt{Santos Small} benchmark, the difference between the systems is less pronounced due to the small value of $k$ (as per the ground truth provided by the authors). Nonetheless, {\sysname} maintains a consistently high precision and recall for all values of $k$. For recall, {\sysname} consistently achieves comparable recall to Starmie and SANTOS. 






\subsubsection{Performance and Scalability Analysis} 
To analyze the cost of achieving our outstanding precision and recall, we analyzed the performance of {\sysname}, Starmie, and SANTOS. For fairness, this analysis is conducted on a single machine because SANTOS and Starmie do not support running on a cluster of machines. Further, we study the preprocessing time, i.e. the offline time required to analyze the tables in a data lake, and the average query time, i.e. the time required to retrieved unionable tables given a query table, averaged over all query tables (see Table \ref{tab:data_discovery_dataset_stats} for the number of query tables for each benchmark). 

Table~\ref{tab:scalability_vs_santos} summarizes our results. {\sysname} consistently outperforms SANTOS and Starmie for preprocessing and average query times for both small and large benchmarks. We focus on the \texttt{SANTOS Large} benchmark as it has the highest number of tables.
{\sysname} is 7.3x times faster than SANTOS in preprocessing time. This is because SANTOS analyzes data lake tables on the granularity of column values, matching each value against two knowledge bases (KB): an open KB (YAGO \cite{yago}), and a synthesized KB generated during preprocessing. SANTOS then iterates over \textit{all value pairs} of matching columns per table to determine their semantic relationships. On the other hand, {\sysname} analyzes data lakes on the granularity of columns, applying CoLR models to samples of columns. Compared to Starmie, {\sysname} achieves a 1.8x speed up in preprocessing time. The preprocessing phase of Starmie includes training a language model (LM) to generate the column embeddings for a data lake. Starmie uses data augmentation on data lake columns to generate enough samples to train the LM. Further, Starmie needs to train the LM for enough number of epochs to achieve a decent score (we use 10 epochs as per the author recommendation). Unlike Starmie, {\sysname} does not require training the CoLR models per data lake to generate column embeddings because our models are independently pre-trained on Kaggle and OpenML datasets. 

\input{tables/scalability}

Furthermore, {\sysname} is designed to scale for discovery queries by leveraging the built-in indices in RDF engines. Compared to SANTOS, {\sysname} is 51.2 times faster on average for the \texttt{SANTOS Large} benchmark. For a query table, SANTOS retrieves a list of candidate unionable tables by looking up two indices (one for each KB) for column relationships similar to those found between pairs of columns in the query table. Then, the query table is matched against candidate tables at different granularities to determine the unionability score for each candidate. This results in a large number of comparison and higher query times for SANTOS. Similarly , {\sysname} is 3.3x faster than Starmie in average query time. While Starmie uses an efficient vector index (Hierarchical Navigable Small World (HNSW) \cite{hnsw}) to retrieve similar columns based on embeddings, it requires calculating an approximate distance between embeddings of size 768. However, a discovery query of {\sysname} takes a table graph node and utilizes efficient RDF indices to find unionable tables, which is significantly faster as shown in Table \ref{tab:scalability_vs_santos}. 
 
 
\subsubsection{{\sysname}' Effectiveness Ablation Study}
We perform an ablation study to understand the contribution of our fine-grained CoLR models to the impressive scores shown in Figure \ref{fig:experiment_precision_recall}. Figure \ref{fig:ablation_study} shows the precision and recall of different KGLiDS configurations on the \texttt{TUS Small} benchmark. The highest scores were achieved by utilizing both the CoLR and label embeddings (indicated by the solid line). While column names are a strong predictor of table unionability for the shown benchmarks, raw value-based unionability is useful for data lakes without column names (e.g. anonymized). Figure \ref{fig:ablation_study} illustrates that KGLiDS still performs competitively when using only CoLR embeddings, i.e. predicting unionability based only on raw values.  

\begin{figure}[t]
\vspace*{-2ex}
\centering
\includegraphics[width=\columnwidth]{figures/unionability_ablation_study.pdf} 
\vspace*{-5ex}
  \caption{Ablation study for the effectiveness of {\sysname} for table union search on the \texttt{TUS Small} benchmark.}
  \label{fig:ablation_study}
  \vspace*{-2ex}
\end{figure}

Furthermore, the impact of our approach to training CoLR models for seven fine-grained data types is shown. In comparison to the use of three coarse-grained embedding models as suggested by \cite{MuellerS19}, the fine-grained CoLR models yield significantly higher precision and recall, with precision reaching up to 17\% higher and recall up to 50\% higher at $k=60$. Finally, we evaluate the impact of subsampling columns when applying CoLR models as described in Section \ref{sec:data_profiling}. As shown, applying CoLR models on column samples of 10\% of the original column sizes performs comparably in both precision and recall to applying them on entire columns. However, our subsampling approach reduces the profiling time for the TUS Small benchmark by 14\%. Similar results to this ablation study are obtained on other benchmarks.







\subsection{Pipeline Graphs: {\sysname} vs General-Purpose Tools}
\label{sec:evaluation-pipelineGraphs}

For AutoML, we evaluate \sysname{} against GraphGen4Code~\cite{graph4code} using KGpip \cite{kgpip}, an AutoML approach that utilizes graph neural networks built on top of pipeline graphs. GraphGen4Code~\cite{graph4code} is a toolkit to generate a knowledge graph for code~\footnote{GrapGen4Code is obtained from \url{https://github.com/wala/graph4code}}. 

We used 67 benchmark tables used by the KGpip \cite{kgpip} system. The datasets pertain to different binary and multi-class classification tasks, are real-world datasets from a diversity of sources and problem domains, and are of enough difficulty for the learning algorithms. Table \ref{tab:graph_analysis} summarizes the graph sizes and analysis times for generating the {\graphname} and GraphGen4Code graphs for the Kaggle pipelines dataset. For a fair comparison, we run the pipeline abstraction of {\sysname} on a single machine. Thanks to the lightweight static code, documentation, and dataset usage analyses employed by {\sysname}, it achieves a graph reduction of more than 82\% in 95\% less time for the same set of pipelines.\shorten


In addition, to evaluate the scalability of {\sysname}'s pipeline abstraction, we collected $13,800$ data science pipeline scripts used in the top $1000$ datasets from Kaggle, which includes $3,775$ tables and $141,704$ columns \footnote{The script to download these datasets is available at {\sysname}' repository}. 
We selected these pipelines and datasets based on the number of users' votes on the Kaggle platform. For each dataset, we select up to 20 most voted Python pipelines. The datasets are related to various supervised and unsupervised tasks in different domains, such as health, economics, games, and product reviews. 


\input{tables/graph_anlaysis}
\input{tables/modelled_aspects}

Furthermore, a breakdown of both graphs by the modelled aspects of data science pipelines is shown in Table \ref{tab:modelled_aspects}. Because the focus of GraphGen4Code is the abstraction of general-purpose code, it captures redundant information when used for data science pipelines.
For example, approximately 30\% of GraphGen4Code models local syntactical script information, namely, \emph{statement location}, \emph{variable names}, and \emph{function parameter order}. Without cleaning these aspects, two pipeline scripts with similar semantics could have dissimilar graphs in GraphGen4Code if e.g. they have different variable names. 
In contrast, {\sysname} captures semantics related primarily to data science, including ones not modelled by GraphGen4Code, such as \emph{dataset reads} that indicate when \texttt{CSV} files are read, or \emph{library hierarchy} that model the structure of functions and classes in a data science library. These aspects are essential for automating data science pipelines, such as discovering pipelines for similar datasets and highly effective libraries. In addition, all nodes in the {\graphname} graph are labeled with an RDF type, a standard requirement when constructing knowledge graphs for facilitating graph queries, building a graph schema, and enabling reasoning by RDF engines.





\subsection{Evaluating Our On-Demand Automation Models}
\label{sec:evaluationDataPrep}


As discussed in Section~\ref{sec:applications}, an important application for \sysname{} is onDemand automation of data cleaning, data transformation, and machine learning modelling using AutoML. In this section, we evaluate \sysname{} against SOTA systems in each one.


\subsubsection{Data Cleaning} 


%For training our GNN models for data cleaning and transformation, we used the top-rated one thousand Kaggle datasets comprising $\sim$3.7k tables, $\sim$140k columns, and $\sim$13k pipelines to train \sysname{}'s data preparation recommendation models and control the quality of our recommendations. 



We compare \sysname{} against the most recent version of Holoclean, a.k.a Aimnet~\cite{aimnet}. Aimnet is a data-cleaning system that uses statistical learning and inference to unify a range of data-repairing methods. We used the eight datasets from an AutoML benchmark~\cite{kgpip} that contained missing values and supplemented them with five datasets from the UCI repository~\cite{uci}. 
Our evaluation process consisted of cleaning these datasets using \sysname{} and \holoclean{} and then training a random forest classifier. We also consider a baseline approach that performs modelling without any data cleaning.%The baseline method faced challenges with datasets, whose IDs are 2, 8, and 13. 

The evaluation metric we use to evaluate on-demand data cleaning includes the F1 scores of the random forest classifier trained using cross-validation over ten folds on the cleaned datasets. We also evaluate the cleaning systems in their efficiency in terms of execution time and memory requirements.

\input{tables/cleaning_results}

Table~\ref{tab:cleaning_results} shows that our system (\sysname{}) has consistently higher F1 scores than \holoclean{}. Cleaning data using \holoclean{} led to a better performance in only one dataset, which had an F1 score above 95 for all systems anyway. 

\begin{figure}[t]
\vspace{-2ex}
  \centering
    \includegraphics[width=\columnwidth]{figures/cleaning_results_new_emb.png}
    \vspace*{-4ex}
    \caption{The performance of {\sysname} in data cleaning in comparison to \holoclean{} (Aimnet) using multiple ML tasks on 13 datasets. The X-axis represents the dataset ID, and the Y-axis is the time and memory used to achieve these results. 
    % (a) {\sysname{}} is the only system capable of completing the task on all datasets and outperforms both the baseline and \holoclean{} in 7 out of the 13 datasets (b) and (c) the time and memory consumed per system to perform data cleaning on the dataset and train the model. 
    \holoclean{} (Aimnet) exceeds the memory budget in datasets $11$, $12$, and $13$. %{\sysname} outperforms in most cases Aimnet in terms of accuracy while consuming less time and almost a fixed amount of memory.
    } 
  \label{fig:exp_data_cleaning}
  \vspace{-2ex}
\end{figure}

Figure \ref{fig:exp_data_cleaning} shows that \sysname{} is outperforming \holoclean{} in $85\%$ of datasets in execution time and in $38\%$  datasets in memory usage. Note that the disadvantage of using more memory diminishes as the dataset gets larger because most of this memory is used by the training graph. %This also shows that \sysname{} can scale to very large datasets. 
For example, \holoclean{} failed with out-of-memory errors while attempting to clean datasets $\#11$, $\#12$, and $\#13$, and could not complete the cleaning process for these datasets\footnote{This is also why the F1 score for \holoclean{} in these datasets is $0$ as shown in Table~\ref{tab:cleaning_results}.}. \holoclean{} generates multiple tables containing dataset information throughout its cleaning process. Therefore, its memory requirements increase as the dataset size increases. In contrast, \sysname{}'s memory requirement is constant because it relies on LiDS graph semantics. %balances between efficiency and cleaning effectiveness, allowing users to clean their datasets effectively with little time and memory constraints.






\subsubsection{Data Transformation} 

We compare \sysname{} against \autolearn{} \cite{autolearn}, a regression-based feature learning algorithm that automates feature engineering.
In this evaluation, we used datasets from~\autolearn{}'s experimental evaluation~\cite{autolearn} which is available in the UCI repository~\cite{uci}. These datasets were assigned IDs from $14$ to $30$. 
Similar to data cleaning, our evaluation process includes applying the data transformation recommended by \sysname{} and \autolearn{} to each dataset and then we trained a random forest classifier.% using a 5-fold cross-validation approach. 

% We probably should delete the following paragraph, or move it to the subsection.
The evaluation metric we use to evaluate on-demand data cleaning includes the F1 scores of the random forest classifier trained using cross-validation over 5-fold on the transformed datasets. We also evaluate the cleaning systems in their efficiency in terms of execution time and memory requirements.

\input{tables/transformation_results}
Table~\ref{tab:transformation_results} shows the accuracy achieved by each system. 


Figure~\ref{fig:transformation_autolearn} shows the execution time and memory usage of each system while transforming each dataset. X-axis is the dataset ID. Consistently with data cleaning results, \sysname{} outperformed its competitor in execution time, while memory usage did not increase dramatically as the data size increases. Overall, \sysname{} outperformed \autolearn{} on $65\%$ of the datasets in F1 score while consuming less time and almost fixed memory w.r.t \autolearn{}. 






\begin{figure}[t]
% \vspace{-2ex}
\centering
\includegraphics[width=\columnwidth]{figures/transformation_autolearn.png} 
\vspace*{-4ex}
  \caption{Data Transformation: the performance of {\sysname} vs. \autolearn{} on multiple ML tasks using 18 datasets. (a) and (b) the time and memory consumed per system to perform data transformation on the dataset. {\sysname} outperforms \autolearn{} in terms of time while memory usage does not significantly increase with large datasets.}
  \label{fig:transformation_autolearn}
  \vspace*{-2ex}
\end{figure}










\subsubsection{AutoML}

We integrated the revised version of the KGpip pipeline into {\sysname}. The inference pipeline utilizes {\graphname} to recommend a starting point for the hyperparameter search. The recommended initial hyperparameters by {\sysname} for a given dataset are the most commonly used for the top-voted pipelines associated with the most similar dataset found in the {\graphname} graph. 
Figure \ref{fig:automl_experiment} shows a comparison in the F-Score of the original KGpip pipeline ($Pip_{G4C}$) using GraphGen4Code and our revised pipeline ($Pip_{LiDS}$) using our {\graphname} graph. We follow the same evaluation procedure in~\cite{kgpip} and limit the time budget to 40 seconds to avoid the exploration of the full search space. 
$Pip_{LiDS}$ outperforms $Pip_{G4C}$ in the majority of datasets, with an absolute difference in F-Score reaching 0.29 in some datasets. In addition, a \textit{two-tailed t-Test} between the scores obtained from both pipelines shows that $Pip_{LiDS}$ has significantly better scores with a t-Test value of $0.012$ ($p < 0.05$). This shows that by using the {\graphname} graph, an AutoML system can directly benefit from the accumulated knowledge of data scientists to improve the score or reduce the time budget required for exploring the hyperparameter search space.\shorten


\begin{figure}[t]
% \vspace*{-2ex}
 \centering
  \includegraphics[width=\columnwidth]{figures/automl_results_vs_graph4_code.pdf} 
  \vspace*{-3ex}
  \caption{F1-Score difference between KGpip with GraphGen4Code and KGpip with KGLiDS on 24 binary and multi-class classification AutoML datasets, where the difference between both systems is $> 0.01$.}
  \label{fig:automl_experiment}
  \vspace*{-2ex}
\end{figure}

% We evaluated the usability of {\sysname} for the problem of automatically generating optimized ML pipelines (AutoML). As described in Section \ref{sec:automl_use_case}, we integrated {\sysname} within KGpip, an AutoML framework that utilizes GraphGen4Code and graph neural networks to generate ML pipelines. We used {\sysname} to generate pipeline graphs for the same training set of KGpip. % This recommendation is formulated as a SPARQL query that executes within 361 milliseconds on average. GraphGen4Code does not maintain information on dataset similarities or pipeline votes and, therefore, cannot provide such a recommendation. 
%
 


==> sections/evaluation-old.tex <==
%!TEX root = ../paper.tex

\section{Experimental Evaluation}
\label{sec:evaluation}


%There is no other holistic system in the literature that combines the semantics of code (data science pipelines) and data. Therefore, it is not possible to evaluate {\sysname}'s performance with any single system. Instead, we evaluate {\sysname} against state-of-the-art (SOTA)systems in four real-world applications, namely, table union search, data cleaning, data transformation, and automated machine learning (AutoML). Our evaluation shows that {\graphname} can achieve competitive accuracy compared to these SOTA systems, which are specifically designed for each task. Furthermore, {\sysname} shows superior efficiency in terms of time and memory.


To empirically evaluate {\sysname}, and because there are no holistic systems combining the semantics of programming scripts and data lakes to the best of our knowledge, we evaluated the usability of {\sysname} in four real-world applications, namely, table union search, data cleaning, data transformation, and automated machine learning (AutoML).
We show that applications and models built using the semantics extracted from the {\graphname} graph achieve competitive scores compared to the state-of-the-art systems specifically designed for the same tasks. 
Furthermore, we evaluate the scalability of {\sysname}.


\nsstitle{Compared Systems.}
We evaluate the four applications built using {\sysname} against state-of-the-art systems specifically designed for the same tasks. 
For table union search, we evaluated {\sysname} against two recent systems that achieve the highest scores in recent benchmarks, namely, Starmie \cite{starmie}, which discovers unionable tables via column embeddings from pre-trained language models, and  SANTOS~\cite{santos}, which uses open and synthesized knowledge bases to match column relationships within tables. 


For data cleaning, we compare \sysname{} against a version of Holoclean called Aimnet~\cite{aimnet}, a data cleaning system that uses statistical learning and inference to unify a range of data repairing methods. For data transformation and feature engineering, we compare \sysname{} against \autolearn{} \cite{autolearn}, a regression-based feature learning algorithm that automates feature engineering. All experiments have been executed on a machine running Ubuntu 22.04.2 LTS, with a 2.40 GHz Intel Core Processor CPU with 16 cores and 567 GB of RAM. 
 
Furthermore, for AutoML, we compare our approach with KGpip \cite{kgpip}, an AutoML approach that utilizes graph neural networks and GraphGen4Code~\cite{graph4code}, a toolkit to generate a knowledge graph for code~\footnote{GrapGen4Code is obtained from \url{https://github.com/wala/graph4code}}. For all compared systems, we used the same configurations and hyperparameters recommended by their authors. 

\input{tables/data_discovery_dataset_stats}

\nsstitle{Benchmark Datasets.}
For each application, we used multiple benchmark datasets to evaluate the effectiveness and scalability of our approach.
First, for table union search, we evaluated the effectiveness using the benchmark data lakes developed by $D^3L$ \cite{d3l}, TUS \cite{Fatemeh18}, and SANTOS \cite{santos}, namely \texttt{$D^3L$ Small}\footnote{\url{https://github.com/alex-bogatu/DataSpiders}}, \texttt{TUS Small}\footnote{\url{https://github.com/RJMillerLab/table-union-search-benchmark}}, and \texttt{SANTOS Small} \footnote{\url{https://github.com/northeastern-datalab/santos}}.
\texttt{$D^3L$ Small} is a collection of 654 real-world tables, where each table in the lake is manually annotated with all other related tables. The other two data lakes are collections of 1,539 and 550 synthetic tables, respectively, generated using random horizontal and vertical partitioning from real-world tables. 
In addition, we evaluated the scalability using \texttt{SANTOS Large}, which contains 11,090 tables without ground truth \cite{santos}. The statistics of these benchmarks are shown in Table \ref{tab:data_discovery_dataset_stats}.




Next, for the AutoML application, we used 67 benchmark tables used by the KGpip \cite{kgpip} system. The datasets pertain to different binary and multi-class classification tasks, are real-world datasets from a diversity of sources and problem domains, and are of enough difficulty for the learning algorithms.
In addition, to evaluate the scalability of {\sysname}' pipeline abstraction, we collected 13,800 data science pipeline scripts used in the top 1000 datasets from Kaggle, which includes \textit{3,775} tables and \textit{141,704} columns \footnote{The script to download these datasets is available at {\sysname}' repository}. 
We selected these pipelines and datasets based on the number of users' votes on the Kaggle platform. For each dataset, we select up to 20 most voted Python pipelines. The datasets are related to various supervised and unsupervised tasks in different domains, such as health, economics, games, and product reviews. 

For training our GNN models for data cleaning and transformation, we used the top-rated one thousand Kaggle datasets comprising $\sim$3.7k tables, $\sim$140k columns, and $\sim$13k pipelines to train \sysname{}'s data preparation recommendation models and control the quality of our recommendations.
For testing all systems, we used a total of {\totalDatasets} \textbf{unseen} datasets, collected from different AutoML benchmarks. A complete list of the {\totalDatasets} datasets including their ID and statistics is available at our {\sysname} repository\footnote{\url{https://github.com/CoDS-GCS/kglids/tree/master/gnn_applications}}.  
%
Each dataset is associated with an ML task. We perform data preparation or feature engineering using one of the systems and then model the task. We consider the model utility score as our primary metric to measure the accuracy of each system. We also consider the time and memory consumed by the system.\shorten





\nsstitle{RDF Engines and Computing Infrastructure.}
We used Stardog version \textit{8.0.0} as an RDF engine to store the {\graphname} graph. 
% We deployed the endpoint, {\sysname}, and GrapGen4Code on the same local machine. 
We used two different settings for our experiments. In the first setting, we used a Linux machine with 16 cores and 90GB of RAM. We used this setting to compare the effectiveness and scalability of {\sysname} with other systems.  
% In the second setting, we used a SPARK cluster of 16 machines, each with 64 GB RAM and 16 cores to construct our dataset graphs. Unlike {\sysname}, none of the other systems are distributed, i.e., do not scale up with multiple machines. Therefore, we used this configuration to demonstrate {\sysname}'s strong scalability (Figure \ref{fig:scalability_test}).


\subsection{{\sysname} vs Data Discovery Systems}
We compared {\sysname} to Starmie \cite{starmie} and SANTOS~\cite{santos} in terms of the effectiveness and scalability of table union search on four benchmark datasets:  \texttt{$D^3L$ Small}, \texttt{TUS Small}, \texttt{SANTOS Small}, and \texttt{SANTOS Large}. 

% We evaluate the effectiveness on the former two datasets and the scalability on the latter.
% used both \texttt{SmallerReal} and \textit{Synthetic} datasets of $D^3L$. Both datasets have an average number of 10.7 columns per table. The average number of rows per table is 12,207 in \texttt{SmallerReal} and 1,908 in \textit{Synthetic}. Thus, \texttt{SmallerReal} is more challenging as each table contains 84\% more real data. We got similar results in both datasets.


\begin{figure}
\vspace*{-2ex}
 \centering
\includegraphics[width=\columnwidth]{figures/smaller_real_and_santos_and_tus_precision_recall_column.pdf} 
\vspace*{-4ex}
  \caption{Average precision and recall of unionable table discovery on all benchmark datasets.}
\label{fig:experiment_precision_recall}  
\vspace*{-2ex}
\end{figure}




\subsubsection{Effectiveness of Table Union Search.}
In an extensive collection of datasets, such as a data lake, one of the data discovery tasks is to find unionable tables. As defined in \cite{d3l, Fatemeh18, santos}, for a certain table $T$, \myNum{i} table unionability is calculated in terms of Precision@k and Recall@k for different values of $k$, where $k$ is the number of desired unionable tables to $T$, and \myNum{ii} precision and recall are calculated as the averages over multiple query tables sampled at random. We use the same values of $k$ (185-, 60-, and 10-) and number of query tables (100, 100, and 50) as in previous works evaluating on \texttt{$D^3L$ Small}, \texttt{TUS Small}, and \texttt{SANTOS Small}, respectively. Note that the first data lake is the most challenging because it was manually annotated rather than synthetically generated, has the highest number of rows per table on average, and has a high number of unionable tables of 110 on average. Therefore, we follow \cite{santos} and evaluate unionability on \texttt{SANTOS Small} only up to \texttt{k = 10}. Furthermore, because SANTOS requires additional manual annotation of intent columns for all tables in the lake, we followed the authors' recommendation of using the first columns as intent columns for \texttt{$D^3L$ Small}.

\input{tables/scalability}

Figure \ref{fig:experiment_precision_recall} shows the average Precision@k and Recall@k for the different systems and benchmarks.
{\sysname} significantly outperforms Starmie and SANTOS in terms of precision and recall on $D^3L$ \texttt{Small} and \texttt{TUS Small}.
This outstanding performance shows the advantage of our CoLR models, which are designed and trained per fine-grained data type. 
% $D^3L$ uses hand-crafted feature vectors, which do not capture all aspects of the columns.
Unlike {\sysname}, Starmie uses column embeddings from pre-trained language models, which work well with textual columns but do not achieve the same accuracy for numerical columns. We analyzed Starmie's individual column matches for $D^3L$ \texttt{Small}, which had 52.2 precision for numerical columns compared to 63.4 for textual columns. In addition, our CoLR models are trained to predict column similarity even with different value distributions, which enhances similarity prediction for real-world benchmarks like $D^3L$ \texttt{Small}. Finally, breaking down similarity prediction in the data lake into 7 smaller fine-grained tasks, one per column data type (Table \ref{tab:data_discovery_dataset_stats}), helps greatly reduce the false-positives of {\sysname}. 

For the \texttt{Santos Small} benchmark, the difference between the systems is less pronounced due to the small value of $k$ (as per the ground truth provided by the authors). Nonetheless, {\sysname} maintains a consistently high precision and recall for all values of $k$. For recall, {\sysname} consistently achieves comparable recall to Starmie and SANTOS. 



\subsubsection{Performance and Scalability Analysis.} 
To analyze the cost of achieving our outstanding precision and recall, we analyzed the performance of {\sysname}, Starmie, and SANTOS. For fairness, this analysis is conducted on a single machine because SANTOS and Starmie do not support running on a cluster of machines. Further, we study the preprocessing time, i.e. the offline time required to analyze the tables in a data lake, and the average query time, i.e. the time required to retrieved unionable tables given a query table, averaged over all query tables (see Table \ref{tab:data_discovery_dataset_stats} for the number of query tables for each benchmark). 

Table~\ref{tab:scalability_vs_santos} summarizes our results. {\sysname} consistently outperforms SANTOS and Starmie for preprocessing and average query times for both small and large benchmarks. We focus on the \texttt{SANTOS Large} benchmark as it has the highest number of tables.
{\sysname} is 7.3x times faster than SANTOS in preprocessing time. This is because SANTOS analyzes data lake tables on the granularity of column values, matching each value against two knowledge bases (KB): an open KB (YAGO \cite{yago}), and a synthesized KB generated during preprocessing. SANTOS then iterates over \textit{all value pairs} of matching columns per table to determine their semantic relationships. On the other hand, {\sysname} analyzes data lakes on the granularity of columns, applying CoLR models to samples of columns. Compared to Starmie, {\sysname} achieves a 1.8x speed up in preprocessing time. The preprocessing phase of Starmie includes training a language model (LM) to generate the column embeddings for a data lake. Starmie uses data augmentation on data lake columns to generate enough samples to train the LM. Further, Starmie needs to train the LM for enough number of epochs to achieve a decent score (we use 10 epochs as per the author recommendation). Unlike Starmie, {\sysname} does not require training the CoLR models per data lake to generate column embeddings because our models are independently pre-trained on Kaggle and OpenML datasets. 

Furthermore, {\sysname} is designed to scale for discovery queries by leveraging the built-in indices in RDF engines. Compared to SANTOS, {\sysname} is 51.2 times faster on average for the \texttt{SANTOS Large} benchmark. For a query table, SANTOS retrieves a list of candidate unionable tables by looking up two indices (one for each KB) for column relationships similar to those found between pairs of columns in the query table. Then, the query table is matched against candidate tables at different granularities to determine the unionability score for each candidate. This results in a large number of comparison and higher query times for SANTOS. Similarly , {\sysname} is 3.3x faster than Starmie in average query time. While Starmie uses an efficient vector index (Hierarchical Navigable Small World (HNSW) \cite{hnsw}) to retrieve similar columns based on embeddings, it requires calculating an approximate distance between embeddings of size 768. However, a discovery query of {\sysname} takes a table graph node and utilizes efficient RDF indices to find unionable tables, which is significantly faster as shown in Table \ref{tab:scalability_vs_santos}.     

% Preprocessing: 
%    - compared to SANTOS, we operate on granularity of columns while they operate on granularity of values. 
%    - Compared to Starmie, our CoLR models are pretrained while they train their model for each data lake
% Query:
%    - compared to SANTOS, they query two indecies (YAGO and Synthesized KB) - compared to Starmie, they query based on  embeddings for all columns in query table (fast but not as fast as query nodes in kglids graph)
%

% To analyze the cost of achieving our outstanding precision and recall, we analyzed the performance of {\sysname}, Starmie, and SANTOS in terms of discovery queries and preprocessing times. Table~\ref{tab:scalability_vs_santos} summarizes our results. For fairness, this analysis is conducted on a single machine because SANTOS and Starmie do not support running on a cluster of machines. {\sysname} is designed to scale for discovery queries by leveraging the built-in indices in RDF engines.
% Compared to SANTOS, {\sysname} is two orders of magnitude faster for both datasets.  

 
 
\subsubsection{{\sysname}' Effectiveness Ablation Study}
We perform an ablation study to understand the contribution of our fine-grained CoLR models to the impressive scores shown in Figure \ref{fig:experiment_precision_recall}. Figure \ref{fig:ablation_study} shows the precision and recall of different KGLiDS configurations on the \texttt{TUS Small} benchmark. The highest scores were achieved by utilizing both the CoLR and label embeddings (indicated by the solid line). While column names are a strong predictor of table unionability for the shown benchmarks, raw value-based unionability is useful for data lakes without column names (e.g. anonymized). Figure \ref{fig:ablation_study} illustrates that KGLiDS still performs competitively when using only CoLR embeddings, i.e. predicting unionability based only on raw values.  

\begin{figure}[t]
\vspace*{-2ex}
\centering
\includegraphics[width=\columnwidth]{figures/unionability_ablation_study.pdf} 
\vspace*{-5ex}
  \caption{Ablation study for the effectiveness of {\sysname} for table union search on the \texttt{TUS Small} benchmark.}
  \label{fig:ablation_study}
  \vspace*{-2ex}
\end{figure}

Furthermore, the impact of our approach to training CoLR models for seven fine-grained data types is shown. In comparison to the use of three coarse-grained embedding models as suggested by \cite{MuellerS19}, the fine-grained CoLR models yield significantly higher precision and recall, with precision reaching up to 17\% higher and recall up to 50\% higher at $k=60$. Finally, we evaluate the impact of subsampling columns when applying CoLR models as described in Section \ref{sec:data_profiling}. As shown, applying CoLR models on column samples of 10\% of the original column sizes performs comparably in both precision and recall to applying them on entire columns. However, our subsampling approach reduces the profiling time for the TUS Small benchmark by 14\%. Similar results to this ablation study are obtained on other benchmarks.




\subsection{Pipeline Graphs: {\sysname} vs General-Purpose Tools}
% \subsection{Pipeline Graphs: Abstraction and Usability}
We compared {\sysname} to GraphGen4Code~\cite{graph4code}, a toolkit to generate code graphs, in terms of usability for AutoML with the KGpip \cite{kgpip} AutoML system, qualitative analysis of the generated graphs, and the scalability of pipeline abstraction.  
%
Table \ref{tab:graph_analysis} summarizes the graph sizes and analysis times for generating the {\graphname} and GraphGen4Code graphs for the Kaggle pipelines dataset. For a fair comparison, we run the pipeline abstraction of {\sysname} on a single machine. Thanks to the lightweight static code, documentation, and dataset usage analyses employed by {\sysname}, it achieves a graph reduction of more than 82\% in 95\% less time for the same set of pipelines.\shorten

\input{tables/graph_anlaysis}
\input{tables/modelled_aspects}

Furthermore, a breakdown of both graphs by the modeled aspects of data science pipelines is shown in Table \ref{tab:modelled_aspects}. Because the focus of GraphGen4Code is the abstraction of general-purpose code, it captures redundant information when used for data science pipelines.
For example, approximately 30\% of GraphGen4Code models local syntactical script information, namely, \emph{statement location}, \emph{variable names}, and \emph{function parameter order}. Without cleaning these aspects, two pipeline scripts with similar semantics could have dissimilar graphs in GraphGen4Code if e.g. they have different variable names. 
In contrast, {\sysname} captures semantics related primarily to data science, including ones not modelled by GraphGen4Code, such as \emph{dataset reads} that indicate when \texttt{CSV} files are read, or \emph{library hierarchy} that model the structure of functions and classes in a data science library. These aspects are essential for automating data science pipelines, such as discovering pipelines for similar datasets and highly effective libraries. In addition, all nodes in the {\graphname} graph are labeled with an RDF type, a standard requirement when constructing knowledge graphs for facilitating graph queries, building a graph schema, and enabling reasoning by RDF engines.




%%%%%%%%%%%%%%%%%%%GNN Models for DC and DT
\input{sections/evalDataPrep}
%%%%%%%%%%%%%%%%%%%End

 


==> sections/evaluation_datasets.tex <==
\subsection{Data Discovery}

Data discovery is the task of identifying joinable and unionable tables among a large collection of tables, i.e. a data lake \cite{d3l}.
Since the {\graphname} graph identifies unionability and joinability relationships between tables and columns, data discovery benchmarks can be used to evaluate the quality of the data global schema.

\subsubsection*{\textbf{Baselines and benchmark datasets:}}
We compare our system with two data discovery baselines, namely, $D^3L$ \cite{d3l} and Aurum \cite{aurum}. 
$D^3L$ extracts features from individual columns such as word embeddings of column names, column value distribution and overlap, and regular expressions of column values.
These features are aggregated per table and a hash-based index (LSH) is used to compute unionability and joinability similarities \cite{d3l}. 
Aurum, on the other hand, constructs an in-memory graph structure, where nodes are columns and edges are relationships between them. Similar to $D^3L$, Aurum identifies unionable and joinable columns using LSH indexes of column features \cite{aurum}.
Unlike these baselines, we use deep learned representations of column values and word embeddings of column names to discover unionable and joinable columns and represent these relationships in an RDF graph containing columns, tables, datasets, and data sources. 
In our evaluation, we use the same experiment configuration and benchmark datasets as $D^3L$ \cite{d3l} to compare the accuracy (referred to as effectiveness in \cite{d3l}) of data discovery in the three systems.
This includes two experiments for table unionability and joinability on two benchmark datasets: 1) \texttt{SmallerReal}: a collection of 654 tables (600MB) from open UK government data for different domains such as business, health, transport, etc. \footnote{Available at: \url{https://github.com/alex-bogatu/DataSpiders.git}}, and 2) \textit{Synthetic}: a collection of 5044 tables (1.1 GB) based on Canadian open government data\footnote{Available at \url{https://github.com/RJMillerLab/table-union-search-benchmark.git}}. Table \ref{tab:data_discovery_dataset_stats} shows the statistics of both datasets. In the following experiments, the reported scores (precision/recall) are the averages over a random sample of 100 query tables for each data point (same as \cite{d3l}).

\input{tables/data_discovery_dataset_stats}



\subsubsection*{\textbf{Table relatedness accuracy:}}
In this experiment, we evaluate the accuracy of {\sysname} in predicting similarity relationships between tables.
Given a data lake and a target table $T$, we calculate Precision@k and Recall@k for different values of $k$, where $k$ is the number of related tables to $T$. To this end, we follow \cite{d3l} in defining true positive as a related table to $T$ returned in the top-$k$, a false positive as a non-related table to $T$ returned in the top-$k$ and a false negative as a related table to $T$ not returned in the top-$k$. 
We calculate average precision and recall for 100 target tables sampled at random without replacement for different values of $k$. 


Figures \ref{fig:experiment_precision_recall_smaller_real} and \ref{fig:experiment_precision_recall_syntheticl} show the precision and recall of table relatedness for all systems on the \texttt{SmallerReal} and \texttt{Synthetic} datasets, respectively.
{\sysname} consistently outperforms $D^3L$ and Aurum for both precision and recall on the \texttt{SmallerReal} dataset.
A similar trend is observed on the \texttt{Synthetic} dataset, though with less difference between the systems.
These results demonstrate the effectiveness of our table unionability relationships by breaking down column data types into sub-types using both a named entity recognition model and pattern matching. This decreases the number of false-positive relationships in these majority string benchmark datasets. The results also show the accuracy of our table similarity score, which considers the number of similar columns and their similarity scores.\shorten


% \begin{figure}
%  \centering
%   \includegraphics[width=\columnwidth]{figures/experiment_precision_recall_smaller_real.pdf} 
%   \caption{Average precision (a) and recall (b) of table relatedness for {\sysname}, $D^3L$, and Aurum on \texttt{SmallerReal} dataset as $k$ increases from 5 to 185.}
%   \label{fig:experiment_precision_recall_smaller_real}
% \end{figure}

\begin{figure}
 \centering
  \includegraphics[width=\columnwidth]{figures/experiment_precision_recall_synthetic.pdf} 
  \caption{Average precision (a) and recall (b) of table relatedness for {\sysname}, $D^3L$, and Aurum on \texttt{Synthetic} dataset as $k$ increases from 5 to 350.}
  \label{fig:experiment_precision_recall_syntheticl}
\end{figure}

\subsubsection*{\textbf{Impact of join paths:}}
A join path starting from a table $S$ is a chain of tables that can be joined on one or more columns to populate $S$ with more columns. 
Therefore, for a target table $T$, tables $\bm{\mathcal{J}}=\{J_1,J_2,...,J_n\}$ on join paths starting from either of the top-$k$ related tables are also promising candidates for being related to $T$.



In this experiment, we evaluate the impact of join paths on the \textit{attribute precision} of the top-$k$ related tables on $T$. 

Given a pair of tables,  attribute precision defines the confidence of relatedness among the attributes. This is calculated by counting the match between attributes of target and the predicted related table as a true positive if as per the provided ground truth, the two attributes are related, and a false positive otherwise. With join paths, this definition is extended to include tables in $\bm{\mathcal{J}}$.
We evaluate the attribute precision with and without considering join paths and average the results for 100 randomly sampled target tables at different values of $k$.\shorten 


Figure \ref{fig:attribute_precision_smallerReal} (a) illustrates the comparison of attribute precision with and without considering join paths on the \texttt{SmallerReal} dataset.
For both the settings i.e. with and without join paths, {\sysname} outperforms Aurum for all values of $k$. Attribute precision with join paths is comparable between {\sysname} and $D^3L$ for lower values of $k$, however, for higher values of $k$ {\sysname} outperforms $D^3L$ with a significantly high margin. This is because 
{\sysname} generates deep embeddings of column values which serve as the basis of generating the \texttt{primary-key-foreign-key} relationships. The quality of the joins is clearly demonstrated as it significantly improves attribute precision when taken into consideration. In addition, Figure \ref{fig:attribute_precision_smallerReal} (b) shows the improvement gained by using deep dataset embeddings to predict join paths.


\begin{figure}
 \centering
  \includegraphics[width=\columnwidth]{figures/attribute_precision_dde.pdf} 
  \caption{(a) The impact of considering join paths for attribute precision on \texttt{SmallerReal} dataset for $k \in [5, 260]$ . (b) Using deep dataset embeddings to detect join paths improves the attribute precision in {\sysname}.}
  \label{fig:attribute_precision_smallerReal}
\end{figure}





==> sections/evaluation_old.tex <==
\section{Experimental Evaluation}

In this section, we present an empirical evaluation of {\sysname}. 
We evaluate the data global schema graph and abstracted pipeline graphs independently as there is no other system, to the best of our knowledge, that combines both aspects.
% \subsection{System and Experiment Configurations}
We generated our {\graphname} graph with the following configuration for the data global schema and pipeline graphs. We set the similarity thresholds $\alpha, \beta, \theta,$ and $ \gamma$ shown in Algorithm \ref{alg:data_items_subgraph} to 0.75, 0.95, 0.90, and 0.60, respectively. 
For pipeline abstraction, we analyzed pipeline scripts in written in the Python language (including Jupyter Notebooks) and analyzed the documentation of the top three Python data science libraries, namely, \texttt{Pandas}, \texttt{Sklearn}, and \texttt{Numpy}.
Our experiments are carried out on an Ubuntu machine with 16 cores and 90GB of RAM. 


\input{sections/evaluation_datasets}

\input{sections/evaluation_pipelines}


==> sections/evaluation_pipelines.tex <==
\subsection{Semantic Pipeline Abstraction}
\label{subsec:pipeline_experiments}
In the following experiments, we evaluate the quality and accuracy of our abstracted pipeline graphs.
As there are no standard benchmark tasks for pipeline abstraction, we analyze the pipeline graphs both qualitatively and quantitatively on four graph classification tasks.
\subsubsection*{\textbf{Baseline and benchmark dataset:}}
We compare our system with GraphGen4Code\cite{graph4code}, a toolkit to generate knowledge graphs for Python code \footnote{GrapGen4Code is obtained from \url{https://github.com/wala/graph4code} as of Dec, 2021}.
The knowledge graph of GraphGen4Code includes representations for abstracted of Python code, library documentation and manuals, and forum discussions about code snippets such as those on \url{StackOverflow.com}.
We evaluate only the subgraph of code abstraction with ours as including other parts would give an unfair advantage to our system in the analysis.


% We compare the two systems\footnote{GraphGen4Code is obtained from \url{https://github.com/wala/graph4code} as of Dec, 2021} on a collection of 1,000 Python data science pipelines for the 11 most voted tabular datasets on Kaggle. 
% The datasets are related to a variety of supervised and unsupervised tasks on different domains such as health, economics, games, reviews, etc. 
% The collected pipelines are the most voted ones for each dataset with a maximum of 100 pipelines per dataset to avoid bias towards popular datasets.
% Some of these pipelines are dedicated to data exploration and analysis (EDA), others focus on building machine learning models (with some data exploration).
% We will make this collection available along with the ground truths for the experiments at: \url{https://github.com/CoDS-GCS/kglids}

% Modified section 
% Why did we use kaggle as dataset?
% We didn't have a baseline so we created one using Kaggle top 1000 datasets.
We compare the two systems on a collection of 13,000 Python data science pipelines from Kaggle for 1,000 datasets.
We selected the pipelines and datasets based on the number of user votes on the platform; that is, for the most voted 1,000 tabular datasets, we select the 20 most voted Python pipelines.
The datasets are related to a variety of supervised and unsupervised tasks on different domains such as health, economics, games, and product reviews. 
%Since some restriction over the kind of pipeline analyzed is applied, mainly Python pipeline, some datasets contains less than the targeted 20 pipelines. However, by choosing the most voted pipeline, we ensured that the information that was gather would bring quality feedback to the system.
Amongst these pipelines, some are dedicated to data exploration and analysis (EDA), others focus on building machine learning models (with some data exploration).
The URLs of the datasets and pipelines along with the ground truths for our experiments are available at: \url{https://github.com/CoDS-GCS/kglids}.
We run both systems on this collection and analyze the resultant abstracted pipeline graphs. 
% End modified section


\subsubsection*{\textbf{Qualitative analysis of abstracted pipelines:}}
\input{tables/graph_anlaysis}
\input{tables/modelled_aspects}
Table \ref{tab:graph_analysis} shows a high-level comparison between the pipeline graphs, including the number of RDF triples (i.e. number of edges), number of unique nodes and edges, and the time taken to analyze the pipelines.
For the same set of pipelines, {\sysname}'s pipeline abstraction results in graphs that are one order of magnitude smaller and at least 20 times faster. This demonstrates the scalability of our system as targeting data science applications results in more compact graphs.
\autoref{tab:modelled_aspects} \Mossad{Calculate percentages in this table} Shows a comparison of the abstracted aspects of data science pipelines and the corresponding numbers and percentages of triples in both {\sysname} and GraphGen4Code.
Some of the essential aspects are common in both abstractions, namely, code flow, data flow, library calls, function parameters, statement text, and column reads.
In addition to having a significantly less number of triples, our abstraction is more rich in some of these aspects.
For instance, thanks to our documentation analysis, our abstraction of function parameters includes implicit parameter names and values not specified by the pipeline author.
Furthermore, GraphGen4Code uses string literals to represent called libraries and columns read, while {\sysname} uses RDF nodes that have a well-structured URI and an RDF type. 
For example, to represent \texttt{pandas.DataFrame()}, GraphGen4Code uses "DataFrame", while in {\sysname} it is represented as \texttt{<http://kglids.org/resource/library/pandas/DataFrame>}
Including these semantics is essential for reasoning over the abstracted graphs.


The semantic pipeline abstraction of {\sysname} includes aspects that are not represented in GraphGen4Code. First, statements that read datasets are linked with the corresponding dataset nodes, which together with column reads increase the connectivity between pipelines graphs. Second, our pipeline abstraction inlcludes representation of library component heirarchy, which is useful for the analysis of libraries in pipelines. Moreover, all nodes in the {\graphname} graph are associated with their RDF type to facilitate reasoning over the graphs.

Similarly, GrpahGen4Code includes information not captured in the {\graphname} graph such as statement location, variable names, and order of function parameters (roughly 34\% of triples).
However, these aspects, while potentially relevant for general-purpose code modelling, represent local information to the pipeline rather than its semantics. 


% As for results, one thing remain constant with \autoref{tab:modelled_aspects}, GraphGen4Code evaluates more element than {\sysname}. This is something that comes into the design of the system. For \texttt{Library Calls}, GraphGen4Code evaluates all calls regardless of their    importance whereas {\sysname} only captures calls that are meaningful to the understanding of the pipelines. For example, if we look at every occurrence of \texttt{print}, we don't extract valuable information from the method. They are therefore left out of the resulting graph. The same thing can be said about \texttt{Data flow}. We keep track of only the variables that are important to the understanding of the pipeline.




% \subsubsection*{\textbf{Modeling accuracy:}}

% {\color{red} hello
% In this experiment, we demonstrate pipeline aspects where {\sysname} benefits from the static code analysis catered for data science applications to generate a more accurate abstraction of pipelines.

% The first aspect is the inferred data types of variables and their associated external libraries. 
% While accurately inferring this information is important, the dynamic nature of Python makes it challenging; for example, the function train\_test\_split at line {\lineTrainTestSplit} in our running example takes an input of one or more DataFrame or Numpy array and returns values of the same type split into training and testing portions. 
% Without specific knowledge about this API, it is not feasible to detect statically the data types of the returned values.
% GraphGen4Code fails in such cases as it detects subsequent calls on the returned values as Sklearn calls, i.e. it incorrectly infers the call in line {\lineWrongDataType} as \texttt{sklearn.train\_test\_split.shape} (\texttt{shape} is a DataFrame API).
% However, with little effort in mining the documentation of popular data science libraries, {\sysname} can reliably detect the return type. 

% The information regarding parameters of methods is another benefit of mining the documentation. For train\_test\_split, the method mention earlier, {\sysname} can extract the values passed as parameters and classify \texttt{X} and \texttt{y} as arrays to be analyzed by the method. Moreover, it also link the 5 other parameters that are accepted by train\_test\_split to the particular node and record their value, in this case, the default values. 
% This degree of analysis is not possible without the knowledge that is found within the documentation and thus gives an edge to {\sysname} over GraphGen4Code.

% {\sysname}, like GraphGen4Code, quantify the flow of data throughout the pipeline. This allows the system to view where the information is used in the pipeline and track it inside the graph.

% % Another aspect is the parameter names for function calls in data science pipelines. 
% % Correctly inferring this information amounts to better semantic modeling of pipelines.
% % Explicitly named parameters (e.g. \texttt{k} in line {\lineEasyParamName}) can be modeled using basic abstract syntax tree analysis of Python. 
% % A more challenging yet common case, however, is the one in line {\lineWrongParamName}, where only the value of the first parameter is passed. 
% % While GraphGen4Code cannot handle such cases, {\sysname} correctly identifies the parameter name (\texttt{n\_estimators} in this case) based on the mined documentation of Sklearn.

% We quantified the accuracy of modeling this aspects in our dataset of collected pipelines. 
% \autoref{fig:experiment_pipeline_accuracy} shows the number of correctly modeled statements in the pipelines, i.e. statements where either systems infers the data type correctly. 
% It is evident from the figure that having a data-science-centric analysis achieves a higher modelling accuracy of semantic pipeline abstractions.


% \begin{figure}
%  \centering
%   \includegraphics[width=0.85\columnwidth]{figures/experiment_pipeline_accuracy.pdf} 
%   \caption{Accuracy of {\sysname} and GraphGen4Code in modeling data types and parameter names of data science pipelines.}
%   \label{fig:experiment_pipeline_accuracy}
   
% \end{figure}

% }

\subsubsection*{\textbf{Pipeline Classification}}
In this section, we present a qualitative evaluation of the quality of the abstracted pipelines in both systems. We propose four graph classification tasks (two binary and two multi-class) on our dataset of the most-voted pipelines on Kaggle. The tasks are examples of useful applications a data scientist might build on top of {\sysname}.

In the first task (T1), pipelines are classified by the high-level objective, which might be either: a) building a machine learning pipeline, e.g. by performing data cleaning/feature engineering, then fitting and evaluating a machine learning model (regression, classification, etc.), or b) Exploratory data analysis (EDA) pipelines, which the objective is to analyze the dataset properties (e.g. distribution, outliers, etc.) and visualize the results without fitting an ML model. In task T2, ML pipelines are further classified by the employed ML technique, which is either: a) classical ML pipeline, where relatively simple techniques like linear regression or random forests are used, or b) deep learning pipelines, where the author builds a neural network model via e.g. Keras, TensorFlow, or PyTorch. In task T3, ML pipelines are classified by the ML task as either a) regression, b) classification or c) clustering. Lastly, in task T4, the pipelines are classified by the business domain of the data science task/dataset. We selected the four most popular domains, which are: a) finance, b) education, c) health, and d) entertainment. The expectation is that based on the pipeline structure, the called libraries within the pipeline, or other pipeline semantics, a graph classification model, given enough signal in the pipeline graph, can determine to a certain extent the pipeline class for each task. These four tasks, while challenging, are examples of interesting applications on top of {\sysname}, since, in data science platforms, such information is rarely available. 
 
The ground truth for these tasks is based on the tags of each pipeline explicitly specified by the pipeline authors. We consider only pipelines that have the relevant tags for each task and ignore pipelines that fall into more than one category for the same task, to ensure each pipeline is associated with exactly one class. For each task, we split the pipelines into training, validation, and testing sets with rations, 80\%, 10\%, and 10\%, respectively. Further, we down-sample the majority class, if any, to account for model bias.

In this experiment, we compare the accuracy of a graph classification model when trained on the abstracted pipeline graphs of both {\sysname} and GraphGen4Code. We train a Deep Graph Convolutional Neural Network (DGCNN) \cite{dgcnn} classification model, which takes as input a pipeline graph and its class/label. Additionally, the model requires for each node the associated node embedding. To this end, we train a structural node embedding model, namely, TransE \cite{transE}, for each pipeline graph (both {\sysname} and GraphGen4Code), separately and feed the trained node embeddings to the DGCNN classifier. We use the same training configuration and hyperparameters when training on {\sysname} or GraphGen4Code.

Table \ref{tab:pipeline_classification} shows the number of pipelines for each task as well as the classification accuracy of the classification model when trained on either system (the baseline accuracy is obtained by predicting the majority class). {\sysname} outperforms GraphGen4Code in X out of 4 tasks and performs comparably in X. This shows the required semantics to differentiate between pipelines based on the pipeline task, technique, or domain are captured well in {\sysname} compared to GraphGen4Code. In summary, the experiments for pipeline abstraction demonstrate that our system outperforms that of GraphGen4Code in terms of the rich semantics, graph size, and graph utility.  




\input{tables/pipeline_classification_experiment}


% \subsubsection{Pipeline Completion}

==> sections/governor-new.tex <==
%!TEX root = ../paper.tex

\section{Capturing Semantics}
\label{sec:governor}

{\sysname} captures the semantics of datasets, associated data science pipelines, and programming libraries. Then, it constructs (i) pipeline graphs, e.g., each pipeline script is abstracted and stored in a separate named graph, (ii) a library graph for all programming libraries used by the abstracted pipelines, and (iii) a dataset graph.\shorten


\begin{figure}[t]
\ncp\ncp
 \centering
  \includegraphics[width=\columnwidth]{figures/kglids_running_example_code.pdf} 
  \ncp\ncp\ncp\ncp\ncp\ncp\ncp\ncp
  \caption{A running example to demonstrate the {\sysname} Pipeline Abstraction. In this pipeline script, a dataset is loaded using Pandas and split into training and testing portions. Then, a random forest classifier is fitted and evaluated.}
  \label{fig:running_example}
  \ncp\ncp\ncp\ncp\ncp\ncp
\end{figure} 

\subsection{The Pipeline and Library Graphs}
A data science pipeline, i.e., code or script, performs one or more data science tasks, e.g., data analysis, visualization, or modelling. The pipeline can be abstracted as a control flow graph, in which code statements are nodes and edges are flows of instructions or data. Pipeline P1, in Figure~\ref{fig:kglids_visualization}, is an abstraction of lines 6-10 in Figure~\ref{fig:running_example}. The objective of pipeline abstraction then is to have a language-independent representation of the pipeline semantics, such as code and data flow within a pipeline, invocations of built-in or third-party libraries, and parameters used in such invocations. 

{\sysname} combines analysis of code, library documentation, and dataset usage to have a rich semantic abstraction capturing the essential concepts in data science pipelines. Algorithm~\ref{alg:pipeline_abstraction} sketches the process. 
The main inputs of Algorithm~\ref{alg:pipeline_abstraction} are a set $S = \{s\}$, where $s$ is a pipeline script, $MD$ metadata of pipelines, such as information about datasets used in the pipeline, pipeline author, 
and $LD$ documentations of programming libraries. The algorithm also maintains the \emph{library graph} for the used libraries and a named graph for each pipeline (lines 2 to 3). Our algorithm divides the pipeline abstraction process into a set of independent jobs (line 5), one per pipeline script creating a named graph (line 7) utilizing static code analysis tools, which are natively supported by several programming languages, such as Python (via, for instance, \texttt{ast}\footnote{\url{https://docs.python.org/3/library/ast.html}}) or R (via, for instance, CodeDepends\footnote{\url{https://cran.r-project.org/web/packages/CodeDepends/}}). 

%utilizing static code analysis tools, which are natively supported by several programming languages, such as Python (via, for instance \texttt{ast}\footnote{\url{https://docs.python.org/3/library/ast.html}} and \texttt{astor}\footnote{\url{https://pypi.org/project/astor/}}) or R (via, for instance, CodeDepends\footnote{\url{https://cran.r-project.org/web/packages/CodeDepends/}}). 

%Each statement corresponds to a variable assignment or a method call. If there are multiple calls in a single line, they will correspond to multiple statements.

For each statement in a script, we store the following: i) \emph{code flow}, i.e., the execution order of statements, ii) \emph{data flow}, i.e., subsequent statements that read or manipulate the same data variable, iii) \emph{control flow type}, i.e., whether the statement occurs in a loop, a conditional, an import, or a user-defined function block, which captures the semantics of how a statement is executed, and iv) \emph{statement text}, i.e., the raw text of the statement as it appears in the pipeline. We discard from our analysis statements that have no significance in the pipeline semantics, such as \texttt{print()}, \texttt{DataFrame.head()}, and \texttt{summary()}.\shorten

\input{algorithms/pipeline_abstraction}

Static code analysis is not sufficient to capture all semantics of a pipeline. For instance, it cannot detect that \texttt{pd.read\_csv()} in line 6 in Figure \ref{fig:running_example} returns a Pandas DataFrame object. 
Algorithm~\ref{alg:pipeline_abstraction} further enriches the static code analysis using the documentation of data science libraries (lines 8 to 13). 
Each statement from static code analysis is enriched by the library it calls, names and values of parameters, including implicit and default ones, and data types of return variables. For each class and method in the documentation, we build a JSON document containing the names, values, and data types of input parameters, including default parameters, as well as their return data types. This analysis enables accurate data type detection for library calls to infer the names of implicit call parameters, such as \texttt{n\_estimators} which is the first parameter in line 13 in Figure \ref{fig:running_example}. Static code analysis cannot support this kind of inference.\shorten 

While performing the documentation analysis, we use and expand the \emph{library graph} capturing methods belonging to classes, sub-packages, etc. (shown in red in Figure \ref{fig:kglids_visualization}). This is useful for deriving exciting insights related to data science programming languages. For example, it helps find which libraries are used more frequently than others. {\sysname}, enable retrieving this kind of insight via SPARQL queries against our LiDS graph. \shorten 
Finally, Algorithm~\ref{alg:pipeline_abstraction} uses \textit{Detected Dataset Usage} nodes to capture connections between pipeline statements and the tables or columns used by the pipelines (lines 14--18). If statement reads a table via \texttt{pandas.read\_csv} (e.g. line 7 in Figure \ref{fig:running_example}) or a column via string indices over DataFrames (e.g. line 8 in Figure \ref{fig:running_example}), such tables or columns are identified as potential reads of actual data. In {\sysname}, the Graph Linker  further investigates the detected dataset usage to link these cases into the datasets graph. That helps tracking the usage of datasets, tables, or columns in different pipelines. 



\subsection{Dataset Graph}
Inspired by~\cite{MuellerS19}, {\sysname} uses deep learning to generate embeddings for columns and tables based on their content. 
To also capture semantics, {\sysname} uses a method based on Word Embeddings~\cite{semantic_model}. 
Given a dataset, it is first decomposed into independent tables, and each table is then decomposed into a set of columns, where most computations are done. Statistics and embeddings for tables are then derived from the ones for columns. 
In the following, we only sketch the implementation and refer the interested reader to the extended version of this paper at the {\sysname}'s repository\footnote{\url{https://gitfront.io/r/CoDS-GCS/Ma9Uz7qkpyqu/kglids/blob/techincal_report.pdf}}.

{\sysname} makes use of PySpark DataFrame to analyze columns, enabling scalability via distributed computation and using fixed-size embeddings to represent columns and infer their types. 
In doing so, {\sysname} inherits the PySpark DataFrame support to handle files of different formats, such as CSV, JSON, and Parquet, and connect to relational DB and NoSQL systems. 
Unlike other systems, KGLiDS breaks down the main data types (numerical, textual, and dates) into fine-grained types based on pattern matching and deep learning methods. For example, Booleans, emails, or postal codes are identified using predefined regular expressions while person, organization, or location names are predicted using named entity recognition (NER) models \cite{ner_model}. 

{\sysname} generates deep dataset embeddings (\emph{DeDE}) for each column based on a sample of its actual values. 
We train the DeDE model to capture similarities between columns. DeDE provides three main advantages to KGLiDS; first, higher accuracy of predicted column content similarities in contrast to standard statistical measures \cite{MuellerS19}. Second, it enables data discovery without exposing the datasets' raw content, which is invaluable in an enterprise setting, where access to the raw data might be restricted. Third, a compact representation of fixed-size embeddings, regardless of the actual dataset size, greatly reduces the storage requirements. 
Two columns have similar embeddings if their raw values have high overlap, have similar distributions, or measure the same variable -- even with different distributions (e.g. \texttt{weight\_in\_kg} is similar to \texttt{weight\_in\_gram}).\shorten 

To actually construct the \emph{datasets graph} and its links to the \emph{pipeline graphs}, {\sysname} constructs a metadata subgraph containing the hierarchy structure of the datasets and statistics collected for each column. 
Then, similarity relationship/edges between nodes (columns and datasets) are created by determining their similarities using predefined thresholds -- the similarity values are captured as metadata of the edges and encoded using RDF-star. The pairwise comparisons between columns are processed in a MapReduce fashion. 
To determine the similarity between columns, we use (i) name similarity (similar column names based on GloVe Word embeddings \cite{glove} and a semantic similarity technique \cite{semantic_model}), (ii) content similarity (similar raw values based on the cosine distance between our DeDE embeddings for columns), (iii) inclusion dependency (numerical columns with similar ranges of values included in one another~\cite{dursch2019inclusion}), and (iv)  primary key and foreign key similarity (columns with high uniqueness and content similarity)


==> sections/interfaces.tex <==
% \section{APIs and Use Cases}
\section{The {\sysname} Interfaces}
\label{sec:interfaces}

The primary users of {\sysname} are data scientists in an open or enterprise setting whose objective is to derive insights from their linked data sources and pipelines.
{\sysname} supports several interfaces to fulfill the different use cases for interacting with the {\graphname} graph. 
Predefined operations are a set of carefully designed APIs covering data scientists' needs. In contrast, ad-hoc queries allow a technical user to benefit from the underlying RDF engine by writing SPARQL queries matching a specialized use case in mind. The results of these interfaces are returned as the widely adopted Pandas DataFrames, allowing {\sysname} to integrate with different data science platforms.
The statistics manager facilitates generating reports and statistics about the entities in the {\graphname} graph and the overall usage of the system. Lastly, Data scientists who build machine learning models using the {\graphname} graph can share their models and insights with the community via the model manager. 

\subsection{Predefined Operations}
Consider a scenario where a data scientist is interested in predicting heart failure in patients. They can rely on the predefined operation supported by {\sysname} that allows seamless integration with a conventional data science pipeline. 

\subsubsection*{\textbf{Search tables based on specific Columns}}
In order to get started, the data scientist would like to perform a keyword search using {\sysname} while having certain keywords in mind. This is made available by the following API:
\begin{verbatim}
search_keywords([['heart', 'disease'], 'patients'])
\end{verbatim}
This essentially performs a regex search on the graph using the conditions that are passed by the user. This API expects conditions as the input that are encapsulated together, where the lists in list are associated by an \texttt{AND} condition, and strings in list are associated by an \texttt{OR} condition. This allows the data scientist to move forward with the most interesting datasets as per their use case (say): \texttt{heart-failure-prediction}, \texttt{heart-failure-clinical-data} and \texttt{world-happiness-report}.

\subsubsection*{\textbf{Discover Unionable Columns}}
the data scientist wants to union the first two datasets to have more rows but are not sure which columns to use out of the large number of columns.
{\sysname} provides support to find a common schema, i.e., columns that could be used to union two tables. This can be expressed as:
\begin{verbatim}
find_unionable_columns(dataset1, table1, dataset2, table2)
\end{verbatim}
As Pandas DataFrame, the user can union the two tables using the recommended common schema by {\sysname}.

\subsubsection*{\textbf{Join Path Discovery}}
with this DataFrame, which is non-existent in the {\graphname} graph, the data scientist wants to join it with the third dataset but they are not directly joinable.
{\sysname} embeds the given DataFrame, finds the most similar 
table in the {\graphname} graph, and finds potential join paths to the target table. {\sysname} discovers intermediate tables, e.g., number of hops, and shows the connection between them. This could be expressed as the following:

\begin{verbatim}
get_path_to_table(df, target_dataset, target_table, hops=2)
\end{verbatim}
{\sysname} discovers join paths between two tables using a SPARQL query. We also support more challenging queries, such as the shortest path between nodes, e.g., tables.
The user can easily use Pandas DataFrame to join the intermediate tables.

\begin{comment}
\subsubsection*{\textbf{Pipeline Discovery}}
...
\end{comment}

\subsubsection*{\textbf{Library Discovery}}
With this dataset, the user would like to build an ML pipeline to predict heart failure. 
They would like first to get familiar with the most used libraries in ML pipelines at their organization. 
They use the API:
\begin{verbatim}
get_top_used_libraries(k=10, task='classification')
\end{verbatim}
where \texttt{k} specifies the number of libraries to return.
{\sysname} uses a SPARQL query to retrieve the libraries used in classification pipelines and returns them sorted by the number of pipelines.

\subsubsection*{\textbf{Pipeline Discovery}}
After reading more about the most used libraries, Pandas, Scikit-learn, and XGBoost, the user is interested to see example pipelines where the following components are called: \texttt{pandas.read\_csv}, \texttt{XGBoost.XGBClassifier}, and \texttt{sklearn.f1\_score}.
They use the API:
\begin{verbatim}
get_pipelines_calling_libraries('pandas.read_csv', 
'XGBoost.XGBClassifier', 'sklearn.metrics.f1_score') 
\end{verbatim}
{\sysname} searches the pipelines using a SPARQL query and returns a list of pipelines matching the criteria along with other pipeline metadata, like number of votes, author, language, etc. 

\subsubsection*{\textbf{Feature Recommendation}}
With the observation that similar datasets have similar pipelines, {\sysname} can serve as a companion for building machine learning pipelines, which consist of feature engineering and model building. 
Having a DataFrame that is non-existent in the {\graphname} graph, a data scientist would like to build an ML classification pipeline for their dataset. First, they get insights on which features (columns) to use with the API: 
\begin{verbatim}
recommend_features_for_task(df, task='classification')
\end{verbatim}
{\sysname} suggests the most successful features in the DataFrame by: a) embedding the given DataFrame using the deep dataset embedding model, b) using the generated embeddings to search the embedding store for the most similar dataset $S$, c) using a SPARQL query to retrieve the features in $S$ that are most used in classification pipelines, and d) returning the matching features in the given DataFrame to the top ones in $S$.

\subsubsection*{\textbf{Classifier Recommendation}}
After applying feature engineering to the recommended features, the user can choose a classification model with the API: 
\begin{verbatim}
recommend_ml_models(df, task='classification')
\end{verbatim}
{\sysname}, a) embeds the given DataFrame, b) uses the generated embeddings to search the embedding store for the most similar dataset $S$, c) finds the top-k pipelines for $S$ by score using a SPARQL query, and d) returns classifiers that appear the most in these pipelines, sorted by the score.
The user selects a particular classifier and now would like to find a promising configuration for the hyperparameters of this classifier. 

\subsubsection*{\textbf{Hyperparameter Recommendation}}
{\sysname} provides the API:
\begin{verbatim}
recommend_hyperparameters(df, model)
\end{verbatim}
{\sysname}, a) embeds the given DataFrame using the deep dataset embedding model, b) uses the generated embeddings to search the embedding store for the most similar dataset $S$, c) uses a SPARQL query to find the most popular parameters for calls of the given classifier in pipelines of $S$, and d) returns the most common values for the hyperparameters of the classifier. The user then trains the classifier using the recommended hyperparameters. {\sysname} has saved the user a significant amount of time in trial-and-error searching for the most promising hyperparameters.  
Note that while the previous operations have similarities with an AutoML system, they are based on search queries over the {\graphname} graph. That said, {\sysname} enables data scientists to collect training set consisting of pipeline graphs and the associated datasets to train a GNN-based AutoML system similar to \cite{kgpip}.






\subsection{Model Manager}
Building machine learning models on top of graphs, especially graph neural networks (GNN), has become a standard practice for graph analytics \cite{gnn_survey}.
Data scientists interacting with {\sysname} would like to automate tasks on top of the {\graphname} graph using GNNs. 
This involves building large collections of labeled training data, training and testing several GNN models, and potentially sharing the successful models and insights back with the community.
With the {\graphname} graph in hand, data scientists can easily build training sets to automate various tasks with GNN models. 
For example, consider a scenario, where a data scientist would like to examine pipelines dedicated to data exploration and visualization. They query the {\graphname} graph for pipelines that are manually labelled by their authors as data exploration, i.e. EDA, but realize that only a small portion of pipelines have such labels. 
They decide to build a GNN-based classifier for unlabeled pipelines to differentiate between EDA and ML pipelines based on the rich semantics captured in the graph.
{\sysname} allows the scientist to build a training set consisting of pipeline graphs along with their labels.

Other examples include building a GNN-based classifier to differentiate between deep learning-based pipelines and classical ML ones. 
% to classify p which we demonstrate in Section \ref{sec:evaluation}, is a graph classification model for pipelines by their task or application domain. Other examples include a graph generation network to automatically generate pipelines (AutoML) or a link prediction model to detect similarities for newly added datasets.
The model manager allows data scientists who developed such models to share them with the community. A model consists of a binary file along with instructions on how to load and use it (metadata). The model manager handles the storage and retrieval of these models. Utilizing these models to query the {\graphname} graph is left for future work.




% \begin{enumerate}
% \item Linked data science: i.e., operations that derive insights based on the links between data sources, pipelines, and libraries. Examples include discovering: regressors that have the highest $R^2$ score for a specific dataset, the most popular Scikit feature engineering technique on a given table, features (columns) of a table that are used the most often in ML pipelines, and the most popular hyperparameters for e.g. SVM and a given dataset. 
% \item Pipelines and libraries: operations include finding: example usage of a certain function (e.g. pandas.DataFrame.apply()), feature engineering techniques that are used the most in combination with RandomForestRegressor, and the most popular ML libraries used (e.g. TensorFlow vs. PyTorch).
% \item Data sources: example operations include discovering unionable or joinable tables to a given one, finding a common schema to union two tables, or finding the shortest join path between two tables.
% \item Dataset embeddings: such as calculating embedding for a given DataFrame, finding its most similar table by content, and performing a top-k similarity search for a table based on embeddings. 

% \end{enumerate}

% \subsection{Ad-hoc Queries}
% While the predefined operations cover a wide range of use cases, some technical users might have a specialized way to interact with {\sysname}. Since the {\graphname} graph is stored in an RDF engine, ad-hoc queries are natively supported via the extensible and highly flexible SPARQL query language. The results are returned as a DataFrame of triples (subject, predicate, object).

==> sections/introduction-Dec1.tex <==
%!TEX root = ../paper.tex

\section{Introduction}
\label{sec:introduction}
Data science is the process of collecting, cleaning, and analyzing structured and unstructured data to derive insights and make predictions. To define appropriate pipelines, data scientists dedicate significant time to data discovery, data preparation, and modeling. Unfortunately, data scientists primarily work in isolation without exchanging knowledge with fellow data scientists working on similar tasks and with similar datasets. Consequently, there is only little to no exchange of knowledge and experiences, a phenomenon referred to as ``tribal knowledge''.  

%Data science is the process of collecting, cleaning, and analyzing structured and unstructured data to derive insights or to build models for predicting particular tasks. 
%To achieve these goals, data science is founded on datasets and the pipelines built on top of them.
%Data scientists dedicate significant time to performing data discovery, preparation, and modelling. They often work in isolation, with no support from previous work performed by fellow data scientists on similar datasets. The knowledge gained by data scientists from developing Data Science Pipelines (DSPs) is often not shared, which leads to a phenomenon called "tribal knowledge". There is a need to establish a culture of collaboration and knowledge-sharing to improve the efficiency and effectiveness of different aspects of DSPs through automation~\cite{KEK}.  

Interestingly, scientists can access valuable pipelines not only within individual companies but also through open machine learning (ML) portals, such as Kaggle~\cite{kaggle} and OpenML~\cite{OpenML}. These platforms offer entry to extensive public repositories containing thousands of datasets and hundreds of thousands of pipelines with ample opportunities for learning and benefit.
%
Hence, if it was possible to learn efficiently from such pipelines, data scientists would no longer be forced to reinvent the wheel and instead be able to focus on solving new and complex problems. 
A crucial prerequisite for realizing this objective of effectively sharing and leveraging the implicit knowledge and experiences embedded in existing data science pipelines~\cite{KEK} is to move beyond the specifics of datasets and pipelines. 
The key is to abstract from these details and, instead, capture their semantics. This approach facilitates overcoming challenges related to differences in data formats (CSJ, JSON, etc.), programming languages, and libraries. 
In the context of this paper, we employ knowledge graphs (KGs) to efficiently capture such semantics, relationships, and dependencies -- both with respect to \emph{datasets} and \emph{pipelines}.

%The DSPs created by data scientists in each enterprise are valuable assets for future projects. Furthermore, open ML portals, such as Kaggle~\cite{kaggle} and OpenML~\cite{OpenML} provide access to public repositories containing thousands of datasets and hundreds of thousands of DSPs. The wealth of knowledge available at these repositories can be leveraged to improve the efficiency and accuracy of DSPs and facilitate collaboration and knowledge-sharing among data scientists. By building upon the insights and learnings gained from existing DSPs, data scientists can avoid reinventing the wheel and instead focus on solving new and complex problems. However, these large repositories contain heterogeneous datasets and pipelines, i.e., datasets in different formats (CSV or JSON) and pipeline scripts written in different languages and libraries. Hence, it is difficult to navigate this vast amount of knowledge to explore or automatically learn from relevant pipelines applied to similar datasets. Knowledge Graphs (KG) that represent datasets and DSPs can help enterprises stay at the forefront of data science innovation % and drive more excellent value from the experience gained by their data scientists. 
%by reducing data scientists' overhead in exploring datasets and experimenting with models from scratch.\shorten


\begin{figure*}[t]
\vspace*{-2ex}
 \centering
  \includegraphics[width=\textwidth]{figures/kglids_architecture.pdf} 
  \vspace*{-4ex}
  \caption{An overview of {\sysname}'s main components and the interaction with data sources and pipeline scripts managed by different data science platforms. Data science pipelines and the associated datasets are analyzed via the Pipeline Abstraction and Data Profiling components, respectively. The KG Builder consumes their outputs to construct the {\graphname} graph and maintains the graph and associated embeddings into an RDF-star and embedding stores. Different users can interact with {\sysname} via the {\sysname} Interfaces to extract information or to share with the community their models developed on top of the {\graphname} graph.\shorten}
  \label{fig:overview}
  \vspace*{-3ex}
\end{figure*}
% \end{itemize}

Overall, we identify two streams of related work (dataset search and pipeline generation/recommendation), which have so far been considered separately. To the best of our knowledge, KGLiDS is the first approach to combine these two perspectives within a single holistic framework.
Hence, existing data discovery systems~\cite{starmie, santos, d3l, aurum, Fatemeh18, ZhuDNM19} and data science platforms do not capture the semantics of data science artifacts or interlink the semantics of datasets in data lakes with their corresponding semantics of pipeline scripts available in code repositories~\cite{KEK}. 
While there are several systems recommending data preparation operations, such as exploratory data analysis (EDA)~\cite{dataprep}, data transformations~\cite{autolearn, lfe}, or data cleaning~\cite{aimnet, HoloClean, DataWig, kindi2021}, these systems perform excessive analysis on the raw datasets. Hence, they are computationally expensive and suffer limited scalability with large datasets. Furthermore, Auto-Suggest~\cite{Auto-Suggest} learns from a collection of data science notebooks to recommend operations, such as Join, Pivot, Unpivot, and GroupBy -- but does not offer support for more complex tasks. AutoML systems, such as~\cite{autosklearn, flaml}, learn to predict mainly a classifier and perform hyper-parameter tuning. 
Nevertheless, these systems are limited to analyzing raw datasets and code and therefore cannot capture and exploit the semantics of data science artifacts. 

%Existing data discovery systems~\cite{starmie, santos, d3l, aurum, Fatemeh18, ZhuDNM19} and data science platforms do not capture the semantics of data science artifacts or interlink the semantics of datasets in data lakes with their corresponding semantics of pipeline scripts available in code repositories~\cite{KEK}. 
%% Existing platforms, such as Google Dataset Search, or enterprise data catalog tools, such as Amundsen\cite{amundsen}, offer a rudimentary form of searching for relevant datasets based on keyword matching. 
%% Other state-of-the-art data discovery approaches, e.g., for measuring table relatedness \cite{ZhangI20}, identifying joinable \cite{ZhuDNM19} or unionable \cite{Fatemeh18} tables, work in isolation from each other and do not support discovery based on a combination of diverse features.
%%
%There are several systems recommending data preparation operations, such as exploratory data analysis (EDA)~\cite{dataprep}, data transformations~\cite{autolearn, lfe}, or data cleaning~\cite{aimnet, HoloClean, DataWig, kindi2021}. These systems perform excessive analysis on the raw datasets. Hence, they are computationally expensive and suffer limited scalability with large datasets. Furthermore, Auto-Suggest~\cite{Auto-Suggest} learns from a collection of data science notebooks to recommend operations, such as Join, Pivot, Unpivot, and GroupBy. AutoML systems, such as~\cite{autosklearn, flaml}, learn to predict mainly a classifier and perform hyper-parameter tuning. They may include data pre-processing by analyzing the raw data. These existing systems depend on analyzing raw datasets and do not use the semantics of data science artifacts.\shorten

Although there are a few techniques~\cite{graph4code, code_ontology, hmm_java_ontology} to provide machine-readable semantic abstractions of software code, the majority of these systems target statically-typed languages such as Java, the vast majority of data science pipelines are written in Python, a dynamic language, for which accurate static analysis is challenging or even infeasible in some cases~\cite{pycg}.
To overcome these challenges, this paper proposes an approach tailored specifically to the requirements of data science pipelines in Python and their particularities

%A number of techniques~\cite{graph4code, code_ontology, hmm_java_ontology} has been proposed to provide machine-readable semantic abstractions of software code. The majority of these systems target statically-typed languages like Java, where accurate static code analysis is feasible. However, the vast majority of data science pipelines are not written in Java but in Python, which makes these approaches inapplicable. For example, over 91\% ($\sim$553,000) of pipelines on Kaggle are written in Python according to the Meta Kaggle dataset. Moreover, even existing approaches for Python code~\cite{graph4code} resort to using general-purpose static code analysis techniques although for a dynamic language, such as Python, accurate static analysis is challenging or even infeasible in some cases~\cite{pycg}. 
%Hence, there is a need for approaches tailored specifically to the requirements of data science pipelines in Python and their particularities. In conclusion, although some techniques have been proposed for dataset and pipeline discovery, they (i) have been studied in isolation, (ii) come with several shortcomings, and (iii) have not been integrated into existing platforms that can be used in practice.\shorten

In this paper, we therefore propose {\sysname}, a fully-fledged platform powered by knowledge graphs capturing the semantics of data science artifacts, including both datasets and pipelines, as well as their interconnections. 
To the best of our knowledge, {\sysname} is the first system to combine both dataset and pipeline discovery in a holistic approach. 
In summary, the contributions of this paper are:

%In this paper, we therefore propose {\sysname}, a fully-fledged platform powered by knowledge graphs capturing the semantics of data science artifacts, including both datasets and pipelines, as well as their interconnections. 
%Figure~\ref{fig:overview} illustrates the overall architecture of {\sysname}. To the best of our knowledge, {\sysname} is the first system to encapsulate both aspects of data science in a single representation. \sysname{} proposes an embedding-based data profiling based on DL techniques. Our profiling generates embeddings based on labels, e.g., names of columns or tables, and content of the dataset, e.g., a table or column, instead of the actual data itself. {\sysname} also proposes a lightweight pipeline abstraction technique augmented semantics of programming documentation and dataset usage. \sysname{} has several trained graph neural network (GNN) models to automate the entire process of data science pipelines, such as data cleaning, data transformation, and AutoML. Our GNN models help data scientists while working with new datasets or new data science problems by recommending the most-suited operations. We formalize data cleaning and transformation as a GNN multi-classification task to predict the most likely operation performed on a given table or column from a predefined set of multiple operations. For example, our predefined set of multiple data cleaning operations includes operations such as Fill, Imputation, Interpolation, and Outlier Detection. \sysname{} predicts the cleaning operation based on the table's embeddings.

%In this paper, we constructed a data science KG from the top-rated $1000$ Kaggle datasets and $13,800$ pipeline scripts with the highest number of votes. We trained our models based on the semantics captured in this KG. We conducted a comprehensive evaluation using 4 data lakes and {\totalDatasets} unseen datasets collected from different data discovery and AutoML benchmarks. 
%% These datasets demand different kinds of data preparation and modelling tasks, where each dataset is associated with an ML task. 
%%
%We use these datasets to compare \sysname{} against the state-of-the-art (SOTA) systems in data discovery, cleaning, transformation, and AutoML. Our experiments show that \sysname{} achieves accuracy comparable to the SOTA methods while significantly surpassing them in processing time and reducing memory usage. Hence, \sysname{} automates different aspects of data science pipelines effectively, handles large-scale datasets and works in an interactive manner.\shorten 

%In summary, the contributions of this paper are:

\begin{itemize}
 \item The first and fully-fledged platform\footnote{The {\sysname} repository, ontology, and datasets can be accessed at \url{https://github.com/CoDS-GCS/kglids}} to automate learning and discovery based on the semantics of data science artifacts (the architecture is described in Section~\ref{sec:overview}).
% \item The first and fully-fledged platform\footnote{
 %The {\sysname} repository, ontology, and datasets can be accessed at \url{https://github.com/CoDS-GCS/kglids}} to automate learning and discovery based on the semantics of data science artifacts; Section~\ref{sec:overview}.

 \item Scalable embedding-based data profiling techniques and fine-grained type inference methods to construct a global representation of datasets (Section~\ref{sec:governor}).
 
 \item Capturing the semantics of data science pipelines at scale with specific support for Python (Section~\ref{sec:governor}).
% \item Scalable embedding-based data profiling techniques and fine-grained type inference methods to construct a global representation of datasets. Plus, capturing the semantics related to data science from pipeline scripts at scale with specific support for Python; Section~\ref{sec:governor}.

 \item A novel formalization and scalable implementation of data cleaning and transformation as GNN classification tasks based on the semantics of data science artifacts and dataset embeddings (Section~\ref{sec:applications}).
% \item A novel formalization of data cleaning and transformation as GNN classification tasks based on the semantics of data science artifacts and dataset embeddings. This formalization enables us to scale to large datasets; Section~\ref{sec:applications}.

 \item A comprehensive evaluation using datasets used in existing benchmarks for data lakes and data discovery, data cleaning, transformation, and code abstraction. Our experiments show the superiority of {\sysname} over related work in these areas in terms of time and memory while achieving comparable or better accuracy (Section~\ref{sec:evaluation}).
% \item A comprehensive evaluation using 4 data lakes and {\totalDatasets} unseen datasets used in benchmarks of SOTA systems in data discovery, such as Starmie~\cite{starmie} and Santos~\cite{santos}, Aimnet~\cite{aimnet} in data cleaning, AutoLearn~\cite{autolearn} in data transformation, and GraphGen4Code~\cite{graph4code} in code abstraction. Our experiments show the superiority of {\sysname} over these systems in terms of time and memory performance while achieving comparable or better accuracy; Section~\ref{sec:evaluation}.
\end{itemize}

% \noindent

% The remainder of this paper is organized as follows. Section~\ref{sec:overview} provides an architecture overview of {\sysname}. Section~\ref{sec:governor} describes our knowledge graph construction process. Section~\ref{sec:applications} demonstrates four real-world data science applications enabled by our approach. Section~\ref{sec:evaluation} discusses the results of our comprehensive evaluation. 

While Section~\ref{sec:related_word} discusses related work Section~\ref{sec:conclusion} concludes the paper.

%The remainder of this paper is organized as follows. Section~\ref{sec:overview} provides an architecture overview of {\sysname}. Section~\ref{sec:governor} describes our knowledge graph construction process. Section~\ref{sec:applications} demonstrates four real-world data science applications built using the {\graphname} graph. Section~\ref{sec:evaluation} discusses the results of our comprehensive evaluation. Sections~\ref{sec:related_word} and~\ref{sec:conclusion} present related work and conclusion.\shorten



==> sections/related-work-nov28-Khaled-Mossad.tex <==
%!TEX root = ../paper.tex

\section{Related Work}
\label{sec:related_word}

{\sysname} is the first platform that includes capturing data and code semantics, supporting data discovery activities, and recommending pipelines for data science. It is the first attempt to implement our vision of linked data science on federated datasets~\cite{KEK}. In this section, we will discuss related work in the literature for these two three areas.

\nsstitle{Capturing data and code semantics} Recently, much attention has been given to the problem of constructing fixed-size, low-dimensional representations for tables. Traditional approaches construct table or column embeddings using feature-based ML models \cite{sato} or deep neural networks \cite{MuellerS19}. {\sysname} generates column embeddings using deep neural networks similar to \cite{MuellerS19} and uses them to predict relationships between data items. More recent approaches such as TURL \cite{turl}, TabTransformer \cite{tabtransformer}, and AutoTUS \cite{autotus} generate table representations using language models. These approaches are orthogonal to the problem we are solving, and {\sysname}'s modular design can easily adopt any new data representations as long as they have an approach to represent columns and tables.   

Using knowledge graphs to support applications that analyze and process source code is typical practice in the literature~\cite{scro,code_ontology,hmm_java_ontology,graph4code}. However, these techniques cannot be easily generalized to data science pipelines due to their heavy reliance on the detailed static analysis of Java, where information such as method input and return types is straightforward to determine. The most recent system for code representation is GraphGen4Code \cite{graph4code}, a toolkit utilizing a tool called WALA~\cite{WALA} for general-purpose static code analysis. Unlike GraphGen4Code, {\sysname} combines static code analysis with library documentation and dataset usage analyses to have a rich semantic abstraction that captures the essential concepts in data science pipelines.

\nsstitle{Data Discovery Systems}
Data discovery systems in the literature typically rely on collecting metadata to guide data navigation and discovery. Starmie \cite{starmie} that uses embeddings from language models with an HNSW \cite{hnsw} index. SANTOS \cite{santos} builds column relationship trees by matching column values against open and synthetic knowledge bases. RONIN~\cite{RONIN}, which builds a hierarchical structure of datasets to facilitate the exploration of data lakes. $D^3L$~\cite{d3l}, which constructs a variety of feature vectors for each column and matches them using hash-based indices. These systems use specific formats to store this metadata, which makes it difficult for other systems to use. {\sysname}, on the other hand, uses KG as a navigational data structure that captures the semantics of datasets and pipelines to enable easy integration with any system. More specifically, unlike most existing discovery systems in the literature~\cite{ZhangI20, ZhuDNM19, Fatemeh18}, {\sysname} enables users to query datasets based on embeddings and combines easily different operations in one pipeline script. These data discovery capabilities have been demonstrated in ~\cite{KGLacDemo}.


\nsstitle{Data Pipeline Automation}
Creating data pipeline code automatically is addressed by several research papers from varying perspectives, proposing different methodologies and tools. Some systems are used to investigate bottlenecks and improve the efficiency of data science pipelines, while others focus on improving the accuracy of the data science model. 

The first category includes the FASCA~\cite{FASCA} framework, which addresses the problem by identifying bottlenecks in machine learning pipelines and auto-generates optimized code to tackle the scalability issues seen with increasing data sizes. ~\cite{hetro-pipeline} offers a way to build data pipelines across heterogeneous execution environments and overcome the need for large amounts of glue code [3]. The Rubin Observatory~\cite{rubin} system enables the automatic integration of independently written science algorithms into a processing pipeline. Finally, Phloem~\cite{Phloem} is a compiler that automatically identifies and uses pipeline parallelism in irregular applications.

\sysname{} is in the second category. Another system in this category is Auto-Pipeline~\cite{autopipeline}. Auto-Pipeline~\cite{autopipeline} uses a by-target approach to automate table manipulation operations such as Join and Group-by. Auto-Pipeline takes the raw data and the target schema as input and then automates the necessary transformations to convert input raw data to the specified target. \sysname{} does not have a target schema it is trying to achieve. Instead, the goal for \sysname{} is to improve the quality of the data science pipelines. Auto-pipeline is complementary to \sysname{} and could be used as a prior step to create the tables that \sysname{} needs to transform for data science.\shorten



==> sections/related_work_old.tex <==
\section{Related Work}
\label{sec:related_word}


To the best of our knowledge, {\sysname} is the first work to have a single representation for both the data and pipeline aspects of data science. We review here works that independently address either of these aspects in isolation of the other.

\subsection*{Data Discovery}
several methods have been proposed to support data discovery on top of data lakes. 
\cite{Fatemeh18} address the problem of identifying unionable tables, i.e. tables that can be combined row-wise to add more samples to a dataset, while \cite{ZhuDNM19} identify joinable tables, i.e. tables that can be combined column-wise to add more features to a dataset. 
Other systems \cite{ZhangI20, d3l, aurum} combine these similarity measures when identifying related tables. 
They rely mainly on collected statistics and metadata about the data items, i.e. columns, tables, and datasets. 
Unlike these systems, {\sysname} employs the use of fixed-size learned representations of datasets, which improves the accuracy of identified similarities, while having a more compact representation for data items.

For modeling identified similarities, \cite{goods} use a key-value store to index metadata; \cite{ZhangI20} use both a relational database and a property graph, while \cite{aurum} leverage an in-memory graph to represent similarities between tables and introduce the Source Retrieval Query Language (SQRL) to enable discovery operations on top of it. 
On the contrary, we represent data items and their relationships as a knowledge graph, a persistent storage format that natively supports a well-established, flexible query language (SPARQL).
{\sysname} supports extensible discovery operations via ad-hoc SPARQL queries, greatly increasing its usability. 
% \Mossad{other relevant works: generic\_abstraction\_for\_data, dice}

\subsection*{Semantic Pipeline Representation}


The use of knowledge graphs to support applications on top of source code has seen much traction in recent years.
Several \cite{scro,code_ontology,hmm_java_ontology,graph4code} have been proposed to provide a semantic representation of source code with knowledge graphs. 
Source Code Representation Ontology \cite{scro} and CodeOntology \cite{code_ontology} propose ontologies and RDF serializations for Java-based on the analysis of source code, bytecode, and/or project dependencies.
\cite{hmm_java_ontology} Use Hidden Markov Models to learn ontology for source code in Java. 
However, these techniques cannot be generalized to data science pipelines due to their heavy reliance on the detailed static analysis of Java, where information such as method input and return types is straightforward to determine.
For dynamic languages like Python, such information among others can only be determined at run time. 
{\sysname} proposes specialized static analysis techniques for the semantic abstraction of data science pipelines to compensate for the limited information available. 

Unlike CodeOntology \cite{code_ontology}, where the code abstraction for all files exist in the same graph (default graph), or GraphGen4Code \cite{graph4code}, where each script is isolated in its own named graph, KGLiDS  proposes a different graph organization. An approach more similar to ours is GraphGen4Code \cite{graph4code}, a static-analysis-based toolkit to generate knowledge graphs for Python, where nodes represent function calls and edges indicate code and data flows between them. Unlike {\sysname}, GraphGen4Code uses string literals to model called libraries. Additionally, calls to external libraries such as \texttt{rdflib}\footnote{\url{https://github.com/RDFLib/rdflib}} or \texttt{pandas}\footnote{\url{https://pandas.pydata.org}}  are enriched with their library documentation and relevant forum discussions like those on StackOverflow.


Unlike GraphGen4Code, the static analysis of {\sysname} is more rich and accurate because it relies on assumptions that generally hold for data science pipelines.  
For instance, {\sysname} assumes that every pipeline is associated with a dataset and uses the collected metadata about that dataset to infer the usage of its columns in the pipeline.
Moreover, {\sysname} uses the standard static analysis components that ship with Python (as opposed to the use of WALA\footnote{\url{https://wala.github.io/}} in GraphGen4Code), allowing also for a more lightweight analysis as we demonstrate in section \ref{sec:evaluation}.
Finally, our pipeline abstraction is more compact since we exclude forum discussions and library documentation information as we consider them irrelevant for the problem at hand. 



==> sections/supplementary_material.tex <==
\clearpage
\appendix

\section*{Supplementary Materials}

\section*{F1-Scores of Table Relatedness}

\begin{figure}[h]
  \centering
  \subfloat[a][\texttt{Smaller Real}]{\includegraphics[width=\columnwidth]{figures/F1_score_smaller_real.pdf}  \label{fig:experiment_f1_smaller_real}} \\
  \subfloat[b][\texttt{Synthetic}]{\includegraphics[width=\columnwidth]{figures/F1_score_synthetic.pdf}  \label{fig:experiment_f1_synthetic}}
  
  \caption{Average F1-Score of table relatedness for {\sysname}, $D^3L$, and Aurum on \texttt{Smaller Real} and \texttt{Synthetic} datasets for different values of $k$.}
  
  \label{fig:experiment_f1}
  
\end{figure}


\section*{SPARQL Queries for Query-Based APIs}

In this section, we provide the corresponding SPARQL queries to the ones mentioned in \autoref{sec:use_cases}. All the following queries using these prefixes:

\begin{lstlisting}
PREFIX kglids: <http://kglids.org/>
PREFIX data: <http://kglids.org/data/>
PREFIX pipeline: <http://kglids.org/pipeline/>
\end{lstlisting}


\subsection*{Finding joinable/unionable tables to a given one}

\begin{lstlisting}
SELECT distinct ?similar_table
WHERE {
    ?col_in_target_table kglids:isPartOf <http://kglids.org/datasnaek.youtube-new/dataResource/CAvideos.csv> . #example table
    ?col_in_target_table data:semanticSimilarity ?col_in_similar_table . # data:pkfk for joinable
    ?col_in_similar_table kglids:isPartOf ?similar_table
}
\end{lstlisting}


\subsection*{Finding a common schema between two tables}

\begin{lstlisting}
SELECT DISTINCT ?col_in_table_1 ?col_in_table_2
WHERE {
    ?col_in_table_1 kglids:isPartOf <http://kglids.org/datasnaek.youtube-new/dataResource/CAvideos.csv> . #example table
    ?col_in_table_2 kglids:isPartOf <http://kglids.org/kaggle/shivamb.netflix-shows/dataResource/netflix_titles.csv> .  # example table
    ?col_in_table_1 data:semanticSimilarity ?col_in_table_2
}
\end{lstlisting}


\subsection*{Finding whether two tables have a join path}

\begin{lstlisting}
ASK
{
 <http://kglids.org/datasnaek.youtube-new/dataResource/CAvideos.csv> 
   data:isJoinableWith+ 
   <http://kglids.org/kaggle/shivamb.netflix-shows/dataResource/netflix_titles.csv> .
}
\end{lstlisting}

\subsection*{Fining pipelines that use a particular module (e.g.RandomForestClassifier)}

\begin{lstlisting}
SELECT DISTINCT ?pipeline
WHERE {
    GRAPH ?pipeline {
        ?statement a pipeline:statement .
        ?statement pipeline:callsLibrary <http://kglids.org/pipeline/library/sklearn/ensemble/RandomForestClassifier>
    }
}
\end{lstlisting}

\subsection*{Discovering common classifiers used with a certain feature selection model}

\begin{lstlisting}
SELECT DISTINCT ?classifier (COUNT(?classifier) AS ?classifier_count)
WHERE {
    GRAPH ?pipeline {
        ?statement_feature_statement a pipeline:statement .
        ?statement_feature_statement pipeline:callsLibrary <http://kglids.org/pipeline/library/sklearn/feature_selection/SelectKBest> .
        ?statement_classifier a pipeline:statement .
        ?statement_classifier pipeline:callsLibrary ?classifier` .
        FILTER(REGEX(STR(?classifier), "classifier", "i"))
    }
}
GROUP BY ?classifier
ORDER BY DESC(?classifier_count)
\end{lstlisting}


\subsection*{Finding the most used sub-packages for a certain library}

\begin{lstlisting}
SELECT ?subpackage (COUNT(?subpackage) AS ?subpackage_count)
WHERE {
    ?subpackage kglids:isPartOf+ <http://kglids.org/pipeline/library/pandas> .
    GRAPH ?pipeline {
        ?statement a pipeline:statement .
        ?statement pipeline:callsLibrary ?subpackage
    }
}
GROUP BY ?subpackage
ORDER BY DESC(?subpackage_count)
\end{lstlisting}



\subsection*{Finding short or long pipelines}

\begin{lstlisting}
SELECT ?pipeline (COUNT(?statement) AS ?statement_count)
WHERE {
    GRAPH ?pipeline {
        ?statement a pipeline:statement .
    }
}
GROUP BY ?pipeline ?statement
HAVING (?statement_count < 100) # short pipelines
ORDER BY ?statement_count
\end{lstlisting}



\subsection*{Finding the top-k used columns (i.e. features) in a specific table}

\begin{lstlisting}
SELECT ?column (COUNT(?column_reading_steatement) AS ?column_reads)
WHERE {
    ?column a data:column .
    ?column kglids:isPartOf <http://kglids.org/datasnaek.youtube-new/dataResource/CAvideos.csv> # example table
    GRAPH ?pipeline {
        ?column_reading_steatement a pipeline:statement .
        ?column_reading_steatement pipeline:reads ?column
    }
}
GROUP BY ?column
ORDER BY DESC(?column_reads)
LIMIT 3
\end{lstlisting}



\subsection*{Finding the most common preprocessings on a specific column}

\begin{lstlisting}
SELECT ?preprocessing_module (COUNT(?statement) AS ?module_use)
WHERE {
    ?preprocessing_module kglids:isPartOf+ <http://kglids.org/pipeline/library/sklearn/preprocessing>
    GRAPH ?pipeline {
        ?statement a pipeline:statement .
        ?statement pipeline:callsLibrary ?preprocessing_module .
        ?statement pipeline:reads <http://kglids.org/kaggle/shivamb.netflix-shows/dataResource/netflix_titles.csv/titles> # example column
    }
}
GROUP BY ?preprocessing_module ?statement
ORDER BY DESC(?module_use)
\end{lstlisting}

\subsection*{ Finding common parameter values of a specific classifier (e.g.SVM) on a specific dataset}

\begin{lstlisting}
SELECT ?param_name ?param_value (COUNT(?param_value) AS ?value_count)
WHERE {
    GRAPH ?pipeline {
        ?svm_statement a pipeline:statement .
        ?svm_statement pipeline:callsLibrary <http://kglids.org/pipeline/library/sklearn/svm/SVC> .
        <<?svm_statement pipeline:hasParameter ?param_name>> pipeline:parameterValue ?param_value
    }
}
GROUP BY ?param_name ?param_value
ORDER BY DESC(?value_count)
\end{lstlisting}


==> tables/GNN_specs.tex <==
\begin{table}[t]
\vspace*{-2ex}
  \centering
  \caption{Specifications of the cleaning, scaling and unary recommendation GNN}
  \vspace*{-1ex}
  \label{tab:GNN specs}
  \begin{adjustbox}{width=0.5\textwidth}
    \begin{tabular}{llll}
    \toprule
    Specification & Cleaning model & Scaling model & Unary model \\
    \midrule
   Number of layers & 1 & 1 & 1 \\
   Hidden Channels & 64 & 128 & 64 \\
  Dropout & 0.5 & 0.5 & 0.5 \\
   Learning rate & 0.005 & 0.005 & 0.002 \\
   Epochs & 30 & 30 & 15 \\
   Runs & 3 & 3 & 3 \\
    Batch size & 10000 & 10000 & 10000 \\
    Walk length & 4 & 4 & 4 \\
    Number of steps & 30 & 30 & 10 \\

    \bottomrule
  \end{tabular}
  \end{adjustbox}
\end{table}

==> tables/KGFarm_datasets.tex <==

\begin{table}[ht]
\centering
\caption{Dataset Information}
\begin{adjustbox}{width=0.5\textwidth}
\begin{tabular}{lllllllll}
\hline
Num & Dataset & Size (MB) & \#Rows & \#Columns & \#Categorical & \#Numerical & \%MV & ML Task \\
\hline
1 & hepatitis & 0.01 & 155 & 20 & 0 & 20 & 0.0539 & Classification \\
2 & housevotes84 & 0.02 & 435 & 17 & 17 & 0 & 0.0530 & Classification \\
3 & horsecolic & 0.02 & 300 & 28 & 0 & 28 & 0.1911 & Classification \\
4 & breastcancerwisconsin & 0.02 & 699 & 11 & 0 & 11 & 0.0021 & Classification \\
5 & credit & 0.03 & 690 & 16 & 9 & 7 & 0.0061 & Classification \\
6 & cleveland\_heart\_disease & 0.06 & 303 & 15 & 0 & 15 & 0.0013 & Classification \\
7 & titanic & 0.08 & 891 & 12 & 5 & 7 & 0.0902 & Classification \\
8 & credit-g & 0.16 & 1000 & 21 & 14 & 7 & 0.0037 & Classification \\
9 & jm1 & 1.75 & 10885 & 21 & 0 & 21 & 0.0001 & Classification \\
10 & adult & 5.59 & 48842 & 15 & 9 & 6 & 0.0089 & Classification \\
11 & higgs & 21.69 & 98050 & 29 & 0 & 29 & 3.17E-06 & Classification \\
12 & APSFailure & 99.15 & 76000 & 171 & 1 & 170 & 0.0830 & Classification \\
13 & albert & 256.30 & 425240 & 79 & 0 & 79 & 0.1346 & Classification \\
\hline
13 & Fertility Diagnosis & 0.0125 & 100 & 10 & 9 & 1 & 0 & Classification\\
14 & haberman & 0.0095 & 306 & 4 & 4 & 0 & 0 & Classification\\
15 & wine & 0.0191 & 178 & 14 & 14 & 0 & 0 & Classification\\
16 & ecoli & 0.0584 & 336 & 9 & 7 & 2 & 0 & Classification\\
17 & Pima Indians Subset & 0.0529 & 768 & 9 & 9 & 0 & 0 & Classification\\
18 & dermatology & 0.1157 & 366 & 35 & 34 & 1 & 0.0006 & Classification\\
19 & banknote authentication & 0.0525 & 1372 & 5 & 5 & 0 & 0 & Classification\\
20 & Ionosphere & 0.0939 & 351 & 35 & 35 & 0 & 0 & Classification\\
21 & Sonar & 0.0969 & 208 & 61 & 61 & 0 & 0 & Classification\\
22 & abalone & 0.4861 & 4177 & 9 & 8 & 1 & 0 & Classification\\
23 & libras & 0.2501 & 360 & 91 & 91 & 0 & 0 & Classification\\
24 & waveform & 0.8394 & 5000 & 22 & 22 & 0 & 0 & Classification\\
25 & letter recognition & 3.5478 & 20000 & 17 & 16 & 1 & 0 & Classification\\
26 & optical digits & 2.7872 & 5620 & 65 & 65 & 0 & 0 & Classification\\
27 & feature pixel & 3.6775 & 2000 & 241 & 241 & 0 & 0 & Classification\\
28 & shuttle & 4.4253 & 58001 & 10 & 10 & 0 & 0 & Classification\\
29 & feature Fourier & 1.1751 & 2000 & 77 & 77 & 0 & 0 & Classification\\
30 & poker & 86.0224 & 1025010 & 11 & 11 & 0 & 0 & Classification\\

\hline
\end{tabular}
\end{adjustbox}
\end{table}



==> tables/automl_experiment.tex <==
\begin{table}[]
\caption{F-Scores of the KGpip AutoML system with hyperparameter recommendations from the {\graphname} graph.  the KGpip AutoML system has significantly higher F-Scores on average on 67 benchmark datasets.}
\begin{tabular}{llll}
\toprule
\textbf{\begin{tabular}[c]{@{}l@{}}AutoML\\ Benchmark\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}KGpip+\\ GraphGen4Code\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}KGpip+\\ KGLiDS\end{tabular}} & \textbf{Task} \\
\midrule
albert                    & 0.64                  & \textbf{0.66}         & Binary        \\
blood-transfusion         & \textbf{0.66}         & 0.62                  & Binary        \\
kc1                       & 0.61                  & \textbf{0.67}         & Binary        \\
jm1                       & \textbf{0.57}         & 0.53                  & Binary        \\
APSFailure                & 0.74                  & \textbf{0.84}         & Binary        \\
riccardo                  & \textbf{0.57}         & 0.48                  & Binary        \\
page-blocks               & 0.89                  & \textbf{0.93}         & Binary        \\
cpu\_act\_761             & 0.88                  & \textbf{0.91}         & Binary        \\
airlines                  & 0.55                  & \textbf{0.59}         & Binary        \\
christine                 & 0.69                  & \textbf{0.72}         & Binary        \\
cpu\_small\_735           & 0.84                  & \textbf{0.90}         & Binary        \\
fri\_c1\_1000\_25         & \textbf{0.87}         & 0.83                  & Binary        \\
connect-4                 & 0.26                  & \textbf{0.55}         & Multi-class   \\
jungle\_chess\_2pcs       & \textbf{0.72}         & 0.65                  & Multi-class   \\
vehicle                   & 0.71                  & \textbf{0.77}         & Multi-class   \\
fabert                    & 0.38                  & \textbf{0.67}         & Multi-class   \\
robert                    & 0.32                  & \textbf{0.47}         & Multi-class   \\
cnae-9                    & 0.84                  & \textbf{0.89}         & Multi-class   \\
glass                     & 0.63                  & \textbf{0.66}         & Multi-class   \\
kropt                     & 0.52                  & \textbf{0.69}         & Multi-class   \\
\midrule
Avg. F-Score              & 0.64                  & 0.70                  &       \\
\bottomrule
\end{tabular}
\end{table}




% \begin{table}
% \caption{By using hyperparameter recommendations from the {\graphname} graph, the KGpip AutoML system has significantly higher F-Scores on 6 benchmark datasets.}
% \label{tab:data_discovery_dataset_stats}
% \begin{tabular}{>{\color{blue}}l>{\color{blue}}l>{\color{blue}}l>{\color{blue}}l}
% \toprule
% \begin{tabular}[c]{@{}l@{}}AutoML\\ Dataset\end{tabular}                              & \begin{tabular}[c]{@{}l@{}}KGpip\\ (base)\end{tabular} & \begin{tabular}[c]{@{}l@{}}KGpip+\\ KGLiDS\end{tabular} & Task        \\
% \midrule
% albert                                      & 0.55                & \textbf{0.66}                                           & Binary      \\
% APSFailure                                  & 0.79                & \textbf{0.87}                                           & Binary      \\
% fabert                                      & 0.38                & \textbf{0.67}                                           & Multi-class \\
% robert                                      & 0.32                & \textbf{0.47}                                           & Multi-class \\
% jungle\_chess\_2pcs & 0.75                & \textbf{0.82}                                           & Multi-class \\
% cnae-9                                      & 0.84                & \textbf{0.89}                                           & Multi-class\\
% \midrule
% Avg. F-Score                                & 0.61                & 0.73         &      \\
% \bottomrule
% \end{tabular}
% \end{table}


==> tables/cleaning_transformation_operations.tex <==
% \begin{table}[t]
% \centering
% \caption{Supported cleaning and transformation operations}
% \label{tab:cleaning_trans_operations}
% \begin{tabular}{ll}
% \toprule
% Cleaning Operations        & Fillna, interpolate, KNNImputer, SimpleImputer, IterativeImputer    \\
% Transformation operation     & Sqrt, log, StandardScalaer, MinMaxScaler, RobustScaler   \\
% \bottomrule
% \end{tabular}
% \end{table}

% \begin{table}[t]
% \caption{Supported cleaning and transformation operations}
% \label{table: cleaning_trans_operations}
% \begin{tabular}{p{1.9cm}|p{1.2cm}|p{4.5cm}}
% \toprule
% \multirow{1}{*}{Cleaning} &  & Fillna, Interpolate, KNNImputer, SimpleImputer, IterativeImputer \\
% \hline 

% \multirow{2}{*}{Transformation} & \multirow{1}{*}{Unary} & Log, Sqrt  \\
% \cline{2-3}
% & \multirow{1}{*}{Scaling} &  StandardScalaer, MinMaxScaler, RobustScaler\\

% \bottomrule
% \end{tabular}
% \end{table}

\begin{table}[t]
% \vspace*{-2ex}
\caption{Supported cleaning and transformation operations}
\vspace*{-2ex}
\label{table:cleaning_trans_operations}
\begin{tabular}{p{1.9cm}|p{5.7cm}}
\toprule
\textbf{Cleaning} & Fillna, Interpolate, KNNImputer, SimpleImputer, IterativeImputer \\
\hline 
\textbf{Transformation (Unary)} & Log, Sqrt  \\
\hline
\textbf{Transformation (Scaling)} & StandardScaler, MinMaxScaler, RobustScaler\\
\bottomrule
\end{tabular}
\vspace*{-2ex}
\end{table}


==> tables/modelled_aspects_desc.tex <==
\begin{table*}
\caption{A breakdown of the graphs generated by {\sysname} and GraphGen4Code by the modeled aspects of data science pipelines. The number and percentage of triples modeling each aspect are shown.}
\label{tab:modelled_aspects}
\begin{tabular}{lll|ll|l}
\toprule
Modelled Aspect      & \multicolumn{2}{c}{\sysname} & \multicolumn{2}{c}{GraphGen4Code} & Description                                             \\
\midrule
Dataset reads               & 0.03M      & 00.2\%    &  -        & -      & Table in the data global schema read by a statement e.g. using \texttt{pd.read\_csv()}.            \\
Library hierarchy           & 0.02M      & 00.1\%    &  -        & -      & Hierarchy of library components e.g. \texttt{sum()} part of \texttt{DataFrame} part of \texttt{pandas}.   \\
RDF node types              & 2.55M   & 15.3\%    &   -       & -      & Indicate the RDF type of each node e.g. Dataset, Column, Statement, etc.                                    \\
Statement location          &  -        & -         & 3.97M     & 04.1\% & Starting and ending line and column numbers of statement in the script file.\\
Variable names              &  -        & -         & 0.99M       & 01.0\% & Name of the variable in an assignment e.g. "\texttt{idx}" for the statement: \texttt{idx = 0}.\\
Func. parameter order    &   -       & -         & 25.13M    & 25.8\% & The order in which the parameters of functions are specified (for library calls). \\
Column reads                & 3.52M   & 21.1\%    & 2.00M     & 02.0\% & Column(s) in the data global schema read by each statement.                                \\ 
Library calls               & 0.51M     & 03.0\%    & 15.27M    & 15.6\% &  Calls to external or built-in APIs e.g. \texttt{sklearn.ensemble.RandomForest()}.     \\
Code flow                   & 2.11M   & 12.7\%    & 20.30M    & 20.8\% & Order of execution of code statements.                                      \\
Data flow                   & 1.27M   & 07.6\%    & 13.30M    & 13.6\% & Order of usage of the same data variables (e.g. DataFrame) by code statements.      \\
Control flow type           & 0.81M     & 04.9\%    & 1.12M     & 01.2\% & Special types of code execution e.g. imports, loops, and if-else.                          \\
Func. parameters         & 3.72M   & 22.4\%    & 7.51M     & 07.7\% & Names and values of inferred function parameters (for library calls).                              \\
Statement text              & 2.12M   & 12.7\%    & 7.94M     & 08.1\% & The raw text of a code statement e.g. "\texttt{x = 1}".                                   \\
\midrule
Total                       & 16.64M  & 100\%          & 97.54M    & 100\% &      \\

\bottomrule
\end{tabular}
\end{table*}



% \begin{table*}
% \caption{Number and percentage of triples abstracting different aspects of data science pipelines in {\sysname} and GraphGen4Code.}
% \label{tab:modelled_aspects}
% \begin{tabular}{lll|ll|l}
% \toprule
% Modelled Aspect      & \multicolumn{2}{c}{\sysname} & \multicolumn{2}{c}{GraphGen4Code} & Description                                             \\
% \midrule
% Library call                & 0.51M     & 03.0\%    & 15.27M    & 15.6\% &  \small{Calls to external or built-in APIs e.g. \texttt{sklearn.ensemble.RandomForest()}.}                                       \\
% Code flow                   & 2.11M   & 12.7\%    & 20.30M    & 20.8\% & \small{Order of execution of code statements.}                                       \\
% Data flow                   & 1.27M   & 07.6\%    & 13.30M    & 13.6\% & \small{Order of usage of the same data variables (e.g. DataFrame) by code statements.}       \\
% RDF node types              & 2.55M   & 15.3\%    &   -       & -      & \small{Indicate the RDF type of each node e.g. Statement or Column.}                                    \\
% Control flow type           & 0.81M     & 04.9\%    & 1.12M     & 01.2\% & \small{Special types of code execution e.g. imports, loops, and if-else.}                           \\
% Column reads                & 3.52M   & 21.1\%    & 2.00M     & 02.0\% & \small{Column(s) in the data global schema read by each statement.}                                \\ 
% Dataset reads               & 0.03M      & 00.2\%    &  -        & -      & \small{Table in the data global schema read by a statement e.g. using \texttt{pd.read\_csv()}.}            \\
% Function parameters         & 3.72M   & 22.4\%    & 7.51M     & 07.7\% & \small{Names and values of inferred function parameters (for library calls).}                               \\
% Library hierarchy           & 0.02M      & 00.1\%    &  -        & -      & \small{Hierarchy of library components e.g. \texttt{sum()} part of \texttt{DataFrame} part of \texttt{pandas}.}         \\
% Statement text              & 2.12M   & 12.7\%    & 7.94M     & 08.1\% & \small{The raw text of a code statement e.g. "\texttt{x = 1}".}                                   \\
% Statement location          &  -        & -         & 3.97M     & 04.1\% & \small{Starting and ending line and column numbers of statement in the script file.}\\
% Variable names              &  -        & -         & 0.99M       & 01.0\% & \small{Name of the variable in an assignment e.g. "\texttt{idx}" for the statement: \texttt{idx = 0}.}\\
% Function parameter order    &   -       & -         & 25.13M    & 25.8\% & \small{The order in which the parameters of functions are specified (for library calls).}                                                 \\
% \midrule
% Total                       & 16.64M  &           & 97.54M    & &                                                        \\
% \bottomrule
% \end{tabular}
% \end{table*}


% \begin{table*}
% \caption{Number (in thousands) and percentage of triples abstracting different aspects of data science pipelines in {\sysname} and GraphGen4Code.}
% \label{tab:modelled_aspects}
% \begin{tabular}{lll|ll|l}
% \toprule
% Modelled Aspect      & \multicolumn{2}{c}{\sysname} & \multicolumn{2}{c}{GraphGen4Code} & Description                                             \\
% \midrule
% Library call                & 507.3     & 03.0\%    & 15,272    & 15.6\% &  \small{Calls to external or built-in APIs e.g. \texttt{sklearn.ensemble.RandomForest()}.}                                       \\
% Code flow                   & 2,106.9   & 12.7\%    & 20,304    & 20.8\% & \small{Order of execution of code statements.}                                       \\
% Data flow                   & 1,269.5   & 07.6\%    & 13,295    & 13.6\% & \small{Order of usage of the same data variables (e.g. DataFrame) by code statements.}       \\
% RDF node types              & 2,546.7   & 15.3\%    &   -       & -      & \small{Indicate the RDF type of each node e.g. Statement or Column.}                                    \\
% Control flow type           & 808.8     & 04.9\%    & 1,124     & 01.2\% & \small{Special types of code execution e.g. imports, loops, and if-else.}                           \\
% Column reads                & 3,516.5   & 21.1\%    & 1,997     & 02.0\% & \small{Column(s) in the data global schema read by each statement.}                                \\ 
% Dataset reads               & 26.2      & 00.2\%    &  -        & -      & \small{Table in the data global schema read by a statement e.g. using \texttt{pd.read\_csv()}.}            \\
% Function parameters         & 3,719.6   & 22.4\%    & 7,511     & 07.7\% & \small{Names and values of inferred function parameters (for library calls).}                               \\
% Library hierarchy           & 18.1      & 00.1\%    &  -        & -      & \small{Hierarchy of library components e.g. \texttt{sum()} part of \texttt{DataFrame} part of \texttt{pandas}.}         \\
% Statement text              & 2,120.7   & 12.7\%    & 7,944     & 08.1\% & \small{The raw text of a code statement e.g. "\texttt{x = 1}".}                                   \\
% Statement location          &  -        & -         & 3,972     & 04.1\% & \small{Starting and ending line and column numbers of statement in the script file.}\\
% Variable names              &  -        & -         & 987       & 01.0\% & \small{Name of the variable in an assignment e.g. "\texttt{idx}" for the statement: \texttt{idx = 0}.}\\
% Function parameter order    &   -       & -         & 25,133    & 25.8\% & \small{The order in which the parameters of functions are specified (for library calls).}                                                 \\
% \midrule
% Total                       & 16,640.4  &           & 97,538    & &                                                        \\
% \bottomrule
% \end{tabular}
% \end{table*}

% \begin{table*}
% \caption{Number and percentage of triples abstracting different aspects of data science pipelines in {\sysname} and GraphGen4Code.}
% \label{tab:modelled_aspects}
% \begin{tabular}{llll}
% \toprule
% Modelled Aspect      & {\sysname} & GraphGen4Code & Description                                             \\
% \midrule
% Library call                & 507.3k (3.8\%)      & 15,272k (15.6\%) &  \small{Calls to external or built-in APIs e.g. \texttt{sklearn.RandomForest()}.}                                       \\
% Code flow                   & 2,106.9k (15.9\%)      & 20,304k (20.8\%) & \small{Order of execution of code statements.}                                       \\
% Data flow                   & 1,269.5k (9.6\%)        & 13,295k (13.6\%) & \small{Order of usage of the same data variables (e.g. DataFrame) by code statements.}                                      \\
% RDF node types                   & 2,560.5k (17.0\%)        &   -       & \small{Indicate the RDF type of each node e.g. Statement or Column.}                                    \\
% Control flow type           & 808.8k \ \ (6.1\%)      & 1,124k \ (01.2\%) & \small{Special types of code execution e.g. imports, loops, and if-else.}                           \\
% Column reads                 & 3,516.5k \ \ (1.6\%)      & 1,997k \ \ \ (02.0\%) & \small{Column(s) in the data global schema read by each statement.}                                \\ 
% Dataset reads               & 26.2k \ \ \ \ (0.2\%)      &  -  & \small{Table in the data global schema read by a statement e.g. using \texttt{pd.read\_csv()}.}                                                \\
% Function parameters         & 3,719.6k \ \ (28.0\%)      & 7,511k \ \ \ (7.7\%) & \small{Names and values of inferred function parameters (for library calls).}                               \\
% Library hierarchy           & 18.1k \ \ (0.0\%)      &  -  & \small{Hierarchy of library components e.g. \texttt{sum()} part of \texttt{DataFrame} part of \texttt{pandas}.}                                              \\
% Statement text              & 2,120.7k (16.0\%)      & 7,944k \ \ \ (8.1\%)  & \small{The raw text of a code statement e.g. "\texttt{x = 1}".}                                   \\
% Statement location          &  -         & 3,972k \ \ \ (4.1\%)  & \small{Starting and ending line and column numbers of statement in the script file.}                                            \\
% Variable names              &  -         & 987k \ \ \ (1.0\%) & \small{Name of the variable in an assignment e.g. "\texttt{idx}" for the statement: \texttt{idx = 0}.}                                              \\
% Function parameter order    &   -        & 25,133k (25.8\%) & \small{The order of each function parameter (for library calls).}                                                 \\
% \midrule
% Total                       & 17,315.7k     & 97,538k &                                                         \\
% \bottomrule
% \end{tabular}
% \end{table*}

==> tables/pipeline_classification_experiment.tex <==

\begin{table}[t]
\ncp\ncp
\caption{
A comparison between {\sysname} and GraphGen4Code in terms of modelling. For each task, we report $a(t)$, where $a$ is the classification accuracy and $t$ is the training time in min.\shorten }
\ncp\ncp\ncp
\label{tab:pipeline_classification}
\setlength\tabcolsep{4pt}
\begin{tabular}{@{}l|llll@{}}
\toprule
\multirow{2}{*}{System} & \multicolumn{2}{c|}{Binary Tasks} & \multicolumn{2}{c}{Multi-class Tasks} \\ \cline{2-5} 
\multicolumn{1}{c|}{} & T1 & T2 & T3 & T4 \\
 \midrule
KGLiDS & 59.8 \small{(14.6)} & \textbf{63.5} \small{(8.8)} & \textbf{45.1} \small{(3.2)} & \textbf{36.7} \small{(6.5)} \\

GraphGen4Code & \textbf{66.1} \small{(69.5)} & 60.9 \small{(39.8)} & 38.7 \small{(13.8)} & 34.8 \small{(19.4)} \\ 
\midrule
Baseline Accuracy & 50.4 & 50.5 & 36.4 & 27.6 \\
No. Pipelines & 1974 & 1188 & 551 & 543 \\ 
\bottomrule
\end{tabular}
\ncp\ncp
\end{table}
